Fibered F-Algebra

The concept of F-algebra and its representation can be extended to an arbitrary bundle. We define operations of fibered F-algebra in fiber. The paper presents the representation theory of of fibered F-algebra as well as a comparison of representation of F-algebra and of representation of fibered F-algebra.

==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{texIntro}{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 84 (1966)
}%

\BiblioItem{texGenRelativity}{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{texGenRelativity}{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{texAffine}{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{texAffine}{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric-affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{texAffine}{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{texAffine}{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\BiblioItem{texAffine}{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%

\BiblioItem{texAffine}{0405.027}
{
Aleks Kleyn,
Reference Frame in General Relativity,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2004)
}%

\BiblioItem{texTidal,texAffine}{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{texTidal,texNewton}{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{texNewton}{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{texNewton}{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric-affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{texLagrange}{Weinberg}
{
Steven Weinberg. The Quantum Theory of Fields. Cambridge university press.
}%

\BiblioItem{texLagrange}{Reinhardt}
{
Greiner Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{texLagrange}{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{texTidal}{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{texTidal}{0405.028}
{
Aleks Kleyn, Metric-Affine Manifold,
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2004)
}%

\BiblioItem{texTidal}{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

\BiblioItem{texTidal}{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{texReferenceFrame,texFiberedAlgebra}{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{texFiberedAlgebra,texTstarMorphism}{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

%\BiblioItem{texBasis}{Shilov}
%{
%Г. Е. Шилов, Математический анализ,
%Функции нескольких вещественных переменных, части 1 - 2,
%М., Наука, 1972
%}%

\BiblioItem{texAffine,texRepresentation,texBasis,texDrcBasis,texVectorSpace,texLinearMap}
{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}%

\BiblioItem{texDrcBasis,texBasis}{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М., Наука, 1974
}%

%\BiblioItem{Kleyn} http://www.geocities.com/aleks\_kleyn/Derivative/Derivative.htm

\BiblioItem{texGenRelativity}{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{texGenRelativity}{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{texGenRelativity}{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{texGenRelativity}{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{texGenRelativity}{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{texGenRelativity}{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{texGenRelativity}{Muller}
{
Holger Muller et al.,
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators,
\href{http://prola.aps.org/searchabstract/PRL/v91/i2/e020401}{Phys. Rev. Lett. 91, 020401} (2003),
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2000)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{texGenRelativity,texTidal}{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{texBiring,texVectorSpace}{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem{texBiring,texVectorSpace}
{q-alg-9705026}
{
I.Gelfand, V.Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{texVectorSpace}{Gelfand Retakh 1991}
{
I. Gelfand and V. Retakh, Determinants of Matrices over Noncommutative Rings, Funct.
Anal. Appl. 25 (1991), no. 2, 91-102
}%

\BiblioItem{texVectorSpace}{Gelfand Retakh 1992}
{
I. Gelfand and V. Retakh, A Theory of Noncommutative Determinants and Characteristic
Functions of Graphs, Funct. Anal. Appl. 26 (1992), no. 4, 1-20
}%

\BiblioItem{texVectorSpace}{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{texVectorSpace}{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

%\BiblioItem{texVectorSpace}{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{texVectorSpace}{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{texReferenceFrame}{math.DG-0412391}
{
Александр Клейн,
Frame Manifold,
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2004)
}%

\BiblioItem{texFiberedAlgebra,texBundleRelation,texTstarMorphism}{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2007)
}%

\BiblioItem{texBundleRelation,texPrefaceRelation}{0702.561}
{
Александр Клейн,
Расслоенная алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

%\BiblioItem{texBasis,texLinearMap}{math.RA-0501237}
%{
%Александр Клейн,
%Векторное пространство над телом,\\
%eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2005)
%}%

\BiblioItem{texPolymodule}{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Skew-Field, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\ifx\PrintBook\Defined
\else
\BiblioItem{texVectorSpace,texFiberedAlgebra}{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2006)
}%
\fi

\BiblioItem{texHomotopy}{q-alg-9705009}
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{texIntro}{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81 (1967)
}%

\BiblioItem{texPrefaceRelation}{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem{texBundleRelation,texPrefaceRelation,texTstarMorphism,texCartesian}
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem{texCartesian}
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{texFiberedAlgebra}{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{texBundleRelation}{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{texCalculus}{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem{texCartesian,texFiberedAlgebra}{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{texCalculus}{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{texCalculus}{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология, Использование вещественных чисел в общей топологии,
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
М. Наука, 1975
}

\BiblioItem{texFiberedAlgebra}{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\CloseBiblio



==> Cartesian.Russian.tex <==
%auto-ignore
\def\texCartesian{}

\ifx\PrintBook\Defined
				\chapter{Декартово произведение расслоений}
\fi
			\section{Расслоение}

Допустим $M$ - многообразие и
\symb{\bundle{\mathcal{E}}pEM}0{bundle}
	\begin{equation}
	\label{eq: bundle, definition}
\ShowSymbol{bundle}
	\end{equation}
расслоение над $M$ со слоем $E$.\footnote{Так как мне придётся иметь
дело с различными расслоениями, я буду
пользоваться следующим соглашением. Для обозначения расслоения и слоя я буду пользоваться одной
и той же буквой в разных алфавитах.}
Символ $\bundle{}pE{}$ означает, что
$E$ является типичным слоем расслоения.
Множество $\mathcal{E}$ является областью определения
отображения $\bundle{}pE{}$.
Множество $M$ является областью значений
отображения $\bundle{}pE{}$.
Мы будем отождествлять непрерывное отображение $\bundle{}pE{}$
и расслоение \eqref{eq: bundle, definition}.
Обозначим через
\symb{\Gamma(\bundle{}pE{})}1{set of sections of bundle}
множество сечений расслоения $\bundle{}pE{}$.

\AddIndex{Декартова степень $A$ множества $B$}{Cartesian power of set}
- это множество \symb{B^A}1{Cartesian power of set}
отображений $f:A\rightarrow B$
(\citeBib{Cohn: Universal Algebra}, стр. 18).
Рассмотрим подмножества $B^A$ вида
\[
W_{K,U}=\{f:A\rightarrow B|f(K)\subset U\}
\]
где $K$ - компактное подмножество пространства $A$,
$U$ - открытое подмножество пространства $B$.
Множества $W_{K,U}$ образуют базис топологии
пространства $B^A$. Эта топология называется
\AddIndex{компактно\hyph открытой топологией}{compact open topology}.
Декартова степень $A$ множества $B$,
снабжённая компактно\hyph открытой топологией называется,
\AddIndex{пространством отображений}{mapping space}
(\citeBib{Maunder: Algebraic Topology}, стр. 213).

Согласно \citeBib{Maunder: Algebraic Topology}, стр. 214
для данных пространств $A$, $B$, $C$, $D$ и
отображений $f:A\rightarrow C$, $g:D\rightarrow B$
мы определим морфизм пространства отображений
\[
g^f:D^C\rightarrow B^A
\]
равенством
\begin{align*}
g^f(h)&=fhg&h:&C\rightarrow D&g^f(h):&A\rightarrow B
\end{align*}
Таким образом, морфизм пространства отображений можно представить
с помощью диаграммы
	\[
\xymatrix{
A\ar[rr]^f\ar[d]_{g^f(h)}&&C\ar[d]^h\\
B&&D\ar[ll]^g
}
	\]

Множество $\Gamma(\mathcal{E})$ является подмножеством
множества $\mathcal{E}^M$.
Поэтому мы можем перенести на множество сечений понятия,
определённые для  пространства отображений.
Множества $W_{K,U}$ мы определим следующим образом
\[
W_{K,U}=\{f\in\Gamma(\mathcal{E})|f(K)\subset U\}
\]
где $K$ - компактное подмножество пространства $M$,
$U$ - открытое подмножество пространства $\mathcal{E}$.

	\begin{remark}
Я пользуюсь стрелкой $\xymatrix{\arp[r]&}$
на диаграмме для обозначения проекции расслоения.
	\qed
	\end{remark}

	\begin{remark}
Я пользуюсь стрелкой $\xymatrix{\ars[r]&}$
на диаграмме для обозначения сечения расслоения.
	\qed
	\end{remark}

Пусть $f$ - морфизм расслоения
$\mathcal{E}$ в $\mathcal{E}'$
	\[
\xymatrix{
\mathcal{E}\arp[d]^{\bundle{}pE{}}\ar[rr]^f
&&\mathcal{E}'\arp[d]^{\bundle{}{p'}{E'}{}}\\
M\ar[rr]^F&&M'
}
	\]
Отображение $F$ называется
\AddIndex{базой отображения}{base of map} $f$.
Отображение называется
\AddIndex{лифтом отображения}{lift of map} $F$.

Если отображение $F$ - биекция, то
отображение $f$ определяет морфизм $f^{F^{-1}}$ пространств сечений
$\Gamma(\bundle{}pE{}))$ в $\Gamma(\bundle{}{p'}{E'}{}))$
\shorthandoff{"}
	\[
\xymatrix{
\mathcal{E}\ar[rr]^f&&\mathcal{E}'
&u'=f^{F^{-1}}(u)=fuF^{-1}\\
M\ars[u]^u="U"\ar[rr]^F&&M'\ars[u]_{u'}="UP"
\ar @{=>}^{f^{F^{-1}}} "U";"UP"
}
	\]%
\shorthandon{"}%
Чтобы доказать непрерывность $u'$, достаточно доказать
непрерывность $F^{-1}$. Но это очевидно, так как $F$
непрерывная биекция.

Если $F=\mathrm{id}$, то $\mathrm{id}^{-1}=\mathrm{id}$.
Поэтому морфизм пространств сечений
мы будем обозначать $f^{\mathrm{id}}$. Очевидно
\[
f^{\mathrm{id}}(u)=fu
\]

\ifx\texFuture\Defined
Прежде всего возникает вопрос. Что мы называем расслоением? Когда
мы говорим о расслоении, мы подразумеваем непрерывность базы и
непрерывность слоя. Если слой имеет дискретную топологию, то мы
называем соответствующее множество не расслоением, а слоением.
Расслоения и слоения очень сильно отличаются, и потому мы
используем различные методы для их изучения.
 
Тем не менее, если отвлечься от топологии слоя, эти объекты имееют
нечто общее. Кроме того, нужно иметь в виду следующее.
\begin{itemize}
\item Алгебра может быть определена не только на непрерывном множестве.
Конечные и дискретные группы, например, важны при изучении
многих геометрических объектов и физических явлений.
\item Фактор множество топологического пространства может оказаться
конечным множеством, тем самым разрушая топологию.
В то же время совсем не очевидно, почему мы не должны
рассматривать подобного рода отношение эквивалентности.
\end{itemize}

На данном этапе для меня топология слоя несущественна, но важна
непрерывность базы. Принимая во внимание высказанные выше соображения,
я не буду делать различия между расслоением и накрытием
и буду называть и то, и другое расслоением.
\fi

			\section{Декартово произведение расслоений}
			\label{section: Cartesian Product of Bundles}
		\begin{remark}
		\label{remark: map to Cartesian product}
Пусть $A_1\times...\times A_n$ является декартовым произведением
множеств $A_1$, ..., $A_n$
\shorthandoff{"}
	\[
\xymatrix{
&A_1\times...\times A_n\ar[rd]^{p_n}\ar[ld]_{p_1}\ar[d]&\\
A_1&...&A_n
}
	\]
\shorthandon{"}
Согласно \citeBib{Serge Lang} отображение
\[
f:A\rightarrow A_1\times...\times A_n
\]
можно представить в форме кортежа
\symb{f=(f_1,...,f_n)}1{map to Cartesian product},
где $f_i=fp_i$
\shorthandoff{"}
	\[
\xymatrix{
A\ar[rr]^f\ar[rd]^{f_1}\ar@/_4pc/[rrrd]^{f_n}
&&A_1\times...\times A_n\ar[rd]^{p_n}\ar[ld]_{p_1}\ar[d]&\\
&A_1&...&A_n
}
	\]
\shorthandon{"}
	 \qed
		\end{remark}

Допустим $\bundle{\mathcal{E}_i}{p_i}{E_i}{M_i}$,
$i=1$, ..., $n$ - семейство расслоений.
Для каждого $i$ пусть задано покрытие $\{U_{i\alpha_i}\}$
базы $M_i$ такое, что для любого $U_{i\alpha_i}$
существует локальная тривиализация $\varphi_{i\alpha_i}$
расслоения $\bundle{}{p_i}{E_i}{}$
\shorthandoff{"}
	\[
\xymatrix{
U_{i\alpha_i}\times E_i\ar[rr]^{\varphi_{i\alpha_i}}
\arp[rd]&&\mathcal{E}_i|_{U_{i\alpha_i}}\arp[ld]\\
&U_{i\alpha_i}
}
	\]
\shorthandon{"}%
	 \begin{definition}
	 \label{definition: Cartesian product of bundle}
Для произвольной точки $x_i\in M_i$ выберем
открытое множество $U_{i\alpha_i}$, $i=1$, ..., $n$ 
такое, что $x_i\in U_{i\alpha_i}$.
Мы можем представить точку множества
$\mathcal{E}_i|_{U_{i\alpha_i}}$
в виде кортежа $(x_i,a_i)$, $x_i\in U_{i\alpha_i}$, $a_i\in E_i$.
Для кортежа $\alpha=(\alpha_1,...,\alpha_n)$ рассмотрим
тривиальное расслоение
\[\bundle{\mathcal{E}_\alpha}{e_\alpha}{}{U_\alpha=U_{1\alpha_1}\times...\times U_{n\alpha_n}}\]
элементами которого являются кортежи $(x_1,...,x_n,a_1,...,a_n)$.
Слоем этого расслоения является декартовым произведением
$\prod_{i=1}^n E_i$.
База расслоения является декартовым произведением
$\prod_{i=1}^n U_{i\alpha_i}$.
	 \qed
	 \end{definition}

Непрерывность проекции этого расслоения следует из
следствия 1 предложения 1
(\citeBib{Bourbaki: General Topology 1}, стр. 59).

Чтобы определить расслоение над многообразием $\prod_{i=1}^nM_i$,
мы должны определить функции склеивания. Пусть заданы
функции склеивания $\psi_{i\alpha_i\beta_i}$
расслоения $\bundle{}{p_i}{E_i}{}$ 
\shorthandoff{"}
	\[
\xymatrix{
U_{i\alpha_i}\times E_i\ar[rr]^{\varphi_{i\alpha_i}}
\ar[d]_{(p_i,\overline{\psi}_{i\alpha_i\beta_i})}
&&\mathcal{E}_i|_{U_{i\alpha_i}}
\ar[d]^{\psi_{i\alpha_i\beta_i}}\\
U_{i\beta_i}\times E_i\ar[rr]^{\varphi_{i\beta_i}}
&&\mathcal{E}_i|_{U_{i\beta_i}}
}
	\]
\shorthandon{"}%
Если $U_\alpha\cap U_\beta\ne\emptyset$, то мы
определим склеивающее отображение, пользуясь диаграммой
\shorthandoff{"}
	\[
\xymatrix{
U_\alpha\times E_1\times...\times E_n
\ar[rr]^{id}
\ar[d]_{(p,\overline{\psi}_{1\alpha_1\beta_1},...,
\overline{\psi}_{n\alpha_n\beta_n})}
&&\mathcal{E}|_{U_\alpha}\ar[d]^{\psi_{\alpha\beta}}\\
U_\beta\times E_1\times...\times E_n
\ar[rr]^{id}
&&\mathcal{E}|_{U_\beta}
}
	\]
\shorthandon{"}

Расслоение
\symb{\bundle{}{p_1}{E_1}{}\times...\times\bundle{}{p_n}{E_n}{}}
0{Cartesian product of bundles, definition 1}
\symb{\bundle{}{\prod_{i=1}^n{p_i}}{E_i}{}}
0{Cartesian product of bundles, definition 2}
\[
\ShowSymbol{Cartesian product of bundles, definition 1}=
\ShowSymbol{Cartesian product of bundles, definition 2}=
\bundle{\mathcal{E}}p{\prod_{i=1}^nE_i}M
\]
называется
\AddIndex{декартовым произведением расслоений}{Cartesian product of bundles}
$\bundle{}{p_i}{E_i}{}$.
Мы будем также говорить, что расслоенное пространство $\mathcal{E}$
является \AddIndex{декартовым произведением расслоенных пространств}
{Cartesian product of total spaces}
$\mathcal{E}_i$ и пользоваться обозначением
\symb{\prod_{i=1}^n{\mathcal{E}_i}}
0{Cartesian product of total spaces, definition 2}
\symb{\mathcal{E}_1\times...\times\mathcal{E}_n}
0{Cartesian product of total spaces, definition 1}
\[
\mathcal{E}=
\ShowSymbol{Cartesian product of total spaces, definition 1}=
\ShowSymbol{Cartesian product of total spaces, definition 2}
\]

		\begin{remark}
		\label{remark: Cartesian product, section}
Согласно замечанию \ref{remark: map to Cartesian product}
сечение декартового произведения расслоений
$\bundle{}{p_1}{E_1}{}\times...\times\bundle{}{p_n}{E_n}{}$
можно представить в виде кортежа сечений $a=(a_1,...,a_n)$.
		\qed
		\end{remark}

Мы будем пользоваться следующими диаграммами для представления декартового произведения расслоений
\shorthandoff{"}
	\[
\xymatrix{
&\mathcal{E}\arp@/^1pc/[rdd]^{p_n}\arp@/_1pc/[ldd]_{p_1}&\\
&\times...\times&\\
M_1&...&M_n
}
\ \ \xymatrix{
\mathcal{E}\arp[dd]^{p_i}_{\prod_{i=1}^n}\\
\\
M_i
}
	\]%
\shorthandon{"}%
На диаграмме стрелки, объединённые знаком $\times$ или $\prod$,
символизируют стрелку, соответствующую проекции расслоения
$\mathcal{E}$. Цель обозначения - показать структуру отображения.

В декартовом произведении расслоений определено произведение любых
двух слоёв. Как мы увидим ниже, такое расслоение воспроизводит структуру базы. Это существенно
ограничивает применимость декартова произведения расслоений.

			\section{Приведенное декартово произведение расслоений}
			\label{section: reduced Cartesian Product of Bundles}

Если расслоения определены над общей базой мы можем изменить определение декартова произведения расслоений.

Допустим $\bundle{\mathcal{E}_i}{p_i}{E_i}M$,
$i=1$, ..., $n$ - семейство расслоений
над многообразием $M$.
Для каждого $i$ пусть задано покрытие $\{U_{i\alpha_i}\}$
базы $M$ такое, что для любого $U_{i\alpha_i}$
существует локальная тривиализация $\varphi_{i\alpha_i}$
расслоения $\bundle{}{p_i}{E_i}{}$
\shorthandoff{"}
	\[
\xymatrix{
U_{i\alpha_i}\times E_i\ar[rr]^{\varphi_{i\alpha_i}}
\arp[rd]&&\mathcal{E}_i|_{U_{i\alpha_i}}\arp[ld]\\
&U_{i\alpha_i}
}
	\]
\shorthandon{"}%
	 \begin{definition}
	 \label{definition: reduced Cartesian product of bundle}
Для произвольной точки $x\in M$ выберем
открытые множества $U_{i\alpha_i}$, $i=1$, ..., $n$ 
такие, что $x\in U_{i\alpha_i}$.
Мы можем представить точку множества
$\mathcal{E}_i|_{U_{i\alpha_i}}$
в виде кортежа $(x,a_i)$, $x\in U_{i\alpha_i}$, $a_i\in E_i$.
Для кортежа $\alpha=(\alpha_1,...,\alpha_n)$ рассмотрим
тривиальное расслоение
$\bundle{\mathcal{E}_\alpha}{p_\alpha}{}{U_\alpha=\bigcap_{i=1}^nU_{i\alpha_i}}$,
элементами которого являются кортежи $(x,a_1,...,a_n)$.
Слоем этого расслоения является декартово произведение
$\prod_{i=1}^n E_i$.
База расслоения является множеством $U_\alpha$.
	 \qed
	 \end{definition}

Согласно определению
построенное расслоение над множеством $U_\alpha$ можно
представить в виде
\[
U_\alpha\times\prod_{i=1}^n E_i
\]
Согласно \citeBib{Bourbaki: General Topology 1}, стр. 58,
если $U$ принадлежит базису топологии пространства $U_\alpha$,
то 
$U\times\prod_{i=1}^n E_i$
принадлежит базису топологии пространства $\mathcal{E}_\alpha$.
Если $U$ открытое множество пространства $M$, то
мы можем представить множество $U$ в виде $U=\cup_{i\in I}U_i$,
где $U_i$ принадлежат базису топологии пространства $M$.
Соответственно, множество
\[
p_\alpha^{-1}(U)=U\times\prod_{i=1}^n E_i
\]
может быть представлено в виде
\[
p_\alpha^{-1}(U)=\bigcup_{i\in I}(U_i\times\prod_{i=1}^n E_i)
\]
и является открытым множеством.
Следовательно, проекция $p_\alpha$ является непрерывным отображением.

Чтобы определить расслоение над многообразием $M$,
мы должны определить функции склеивания. Пусть заданы
функции склеивания $\psi_{i\alpha_i\beta_i}$
расслоения $\bundle{}{p_i}{E_i}{}$ 
\shorthandoff{"}
	\[
\xymatrix{
U_{i\alpha_i}\times E_i\ar[rr]^{\varphi_{i\alpha_i}}
\ar[d]_{(p_i,\overline{\psi}_{i\alpha_i\beta_i})}
&&\mathcal{E}_i|_{U_{i\alpha_i}}
\ar[d]^{\psi_{i\alpha_i\beta_i}}\\
U_{i\beta_i}\times E_i\ar[rr]^{\varphi_{i\beta_i}}
&&\mathcal{E}_i|_{U_{i\beta_i}}
}
	\]
\shorthandon{"}%
Если $U_\alpha\cap U_\beta\ne\emptyset$, то мы
определим склеивающее отображение, пользуясь диаграммой
\shorthandoff{"}
	\[
\xymatrix{
U_\alpha\times E_1\times...\times E_n
\ar[rr]^{id}
\ar[d]_{(p,\overline{\psi}_{1\alpha_1\beta_1},...,
\overline{\psi}_{n\alpha_n\beta_n})}
&&\mathcal{E}|_{U_\alpha}\ar[d]^{\psi_{\alpha\beta}}\\
U_\beta\times E_1\times...\times E_n
\ar[rr]^{id}
&&\mathcal{E}|_{U_\beta}
}
	\]
\shorthandon{"}

Расслоение
\symb{\bundle{}{p_1}{E_1}{}\odot...\odot\bundle{}{p_n}{E_n}{}}
0{reduced Cartesian product of bundles, definition 1}
\symb{\bundle{}{\bigodot_{i=1}^n{p_i}}{E_i}{}}
0{reduced Cartesian product of bundles, definition 2}
\[
\ShowSymbol{reduced Cartesian product of bundles, definition 1}=
\ShowSymbol{reduced Cartesian product of bundles, definition 2}=
\bundle{\mathcal{E}}p{\prod_{i=1}^nE_i}M
\]
называется
\AddIndex{приведенным декартовым произведением расслоений}{reduced Cartesian product of bundles}
$\bundle{}{p_i}{E_i}{}$.
Мы будем также говорить, что расслоенное пространство $\mathcal{E}$
является \AddIndex{приведенным декартовым произведением расслоенных пространств}
{reduced Cartesian product of total spaces}
$\mathcal{E}_i$ и пользоваться обозначением
\symb{\bigodot_{i=1}^n{\mathcal{E}_i}}
0{reduced Cartesian product of total spaces, definition 2}
\symb{\mathcal{E}_1\odot...\odot\mathcal{E}_n}
0{reduced Cartesian product of total spaces, definition 1}
\[
\mathcal{E}=
\ShowSymbol{reduced Cartesian product of total spaces, definition 1}=
\ShowSymbol{reduced Cartesian product of total spaces, definition 2}
\]

		\begin{remark}
		\label{remark: reduced Cartesian product, section}
Согласно замечанию \ref{remark: map to Cartesian product}
сечение приведенного декартового произведения расслоений
$\bundle{}{p_1}{E_1}{}\odot...\odot\bundle{}{p_n}{E_n}{}$
можно представить в виде кортежа сечений $a=(a_1,...,a_n)$.
		\qed
		\end{remark}

Мы будем пользоваться следующими диаграммами для представления приведенного декартового произведения расслоений
\shorthandoff{"}
	\[
\xymatrix{
\mathcal{E}\arp@/^2pc/[dd]^{p_n}\arp@/_2pc/[dd]_{p_1}\\
\odot...\odot\\
M
}
\ \ \xymatrix{
\mathcal{E}\arp[dd]^{p_i}_{\bigodot_{i=1}^n}\\
\\
M
}
	\]%
\shorthandon{"}%
На диаграмме стрелки, объединённые знаком $\odot$,
символизируют стрелку, соответствующую проекции расслоения
$\mathcal{E}$. Цель обозначения - показать структуру отображения.

В приведенном декартовом произведении определено произведение слоёв над заданной точкой.
Это делает структуру произведения богаче.

	 \begin{definition}
	 \label{definition: Cartesian power of bundle}
Для $n\ge 0$ мы определим
\AddIndex{декартову степень расслоения}{Cartesian power of bundle}\footnote{Поскольку я рассматриваю
определение декартовой степени расслоения только в рамках приведенного декартова произведения, я не буду пользоваться
соответствующим прилагательным для степени. Это замечание справедливо для всех последующих
определений, связанных с декартовой степенью расслоения.}
\symb{\bundle{}{p}{E}{}^n}0{Cartesian power of bundle}
\symb{\mathcal{E}^n}0{Cartesian power of total spaces}
\[
\left\{
\begin{array}{lr}
\bundle{}{p}{E}{}^0
=\bundle{M}{id}{}M
& n=0\\
\ShowSymbol{Cartesian power of bundle}
=\bundle{\ShowSymbol{Cartesian power of total spaces}}
{\bigodot_{i=1}^n\bundle{}{p}{E}{}}{}M
&n>0
\end{array}
\right.
\]
	 \qed
	 \end{definition}


==> Fibered.Algebra.Russian.tex <==
%auto-ignore
\def\texFiberedAlgebra{}

\ifx\PrintBook\Defined
				\chapter{Расслоенная \texorpdfstring{$\mathcal{F}$}{F}\Hyph алгебра}
\fi

			\section{Расслоенная \texorpdfstring{$\mathcal{F}$}{F}\Hyph алгебра}

	 \begin{definition}
n\Hyph арная
\AddIndex{операция на расслоении}{operation on bundle}
$\bundle{}pE{}$
- это морфизм расслоений
\[
f:\mathcal{E}^n\rightarrow \mathcal{E}
\]
$n$ - это \AddIndex{арность операции}{arity of operation}.
$0$-арная операция - это сечение расслоения
$\bundle{}pA{}$.
	 \qed
	 \end{definition}

Операция на расслоении может быть представлена диаграммой
\shorthandoff{"}
	\[
\xymatrix{
\mathcal{E}^n\ar[rr]^\omega\arp@/^2pc/[dd]^p\arp@/_2pc/[dd]_p&&\mathcal{E}\arp[dd]^p\\
\bigodot...\bigodot\ar@{=>}@/^1pc/[rr]^\omega &&\\
M\ar[rr]^{id}&&M
}
	\]
\shorthandon{"}

		\begin{theorem}
		\label{theorem: continuity of operation}
Пусть $U$ - открытое множество базы $M$,
и на $U$ существует тривиализация расслоения $\bundle{}pE{}$.
Пусть $x\in M$.
Пусть $\omega$ - $n$\Hyph арная операция на расслоении $\bundle{}pE{}$ и
\[
\omega(p_1,...,p_n)=p
\]
в слое $E_x$.
Тогда существуют открытые множества $V\subseteq U$,
$W\subseteq E$, $W_1\subseteq E_1$, ..., $W_n\subseteq E_n$
такие, что $x\in V$, $p\in W$, $p_1\in W_1$, ..., $p_n\in W_n$,
и для любых $x'\in V$, $p'\in W\cap\omega V$ существуют
$p'_1\in W_1$, ..., $p'_n\in W_n$ такие, что
\[
\omega(p'_1,...,p'_n)=p'
\]
в слое $E_{x'}$.
%Если множества $V$, $W$ связны,
%то также связны множества $W_1$, ..., $W_n$.
		\end{theorem}
		\begin{proof}
Согласно \citeBib{Bourbaki: General Topology 1}, стр. 58,
множества вида $V\times W$, где $V$ принадлежит базису
топологии пространства $U$ и $W$ принадлежит базису топологии пространства $E$,
образуют базис топологии пространства $\mathcal{E}$. 
Аналогично множества вида $V\times W_1\times ...\times W_n$, где $V$ принадлежит базису
топологии пространства $U$ и $W_1$, ..., $W_n$ принадлежат базису топологии пространства $E$,
образуют базис топологии пространства $\mathcal{E}^n$. 

Так как отображение $\omega$ непрерывно, то для открытого множества
$V\times W$ существует открытое множество $S\subseteq \mathcal{E}^n$ такое,
что $\omega S\subseteq V\times W$.
Пусть $x'\in V$.
Выберем произвольную точку
$(x',p')\in\omega S$. Тогда существуют такие $p'_1\in E_{x'}$, ..., $p'_n\in E_{x'}$,
что
\[
\omega(p'_1,...,p'_n)=p'
\]
в слое $E_{x'}$.
Согласно сказанному выше существуют множества $R$, $R'$,
принадлежащие базису топологии пространства $U$,
и множества $T_1$, ..., $T_n$,
$T'_1$, ..., $T'_n$, принадлежащие базису топологии пространства $E$,
такие, что $x\in R$, $x'\in R'$,
$p_1\in T_1$, $p'_1\in T'_1$, ..., $p_n\in T_n$, $p'_n\in T'_n$,
$R\times T_1\times ...\times T_n\subseteq S$,
$R'\times T'_1\times ...\times T'_n\subseteq S$.
Теорема доказана, так как
$W_1=T_1\cup T'_1$, ..., $W_n=T_n\cup T'_n$
- открытые множества.
%
%Если $V$ и $W$ связны, то $V\times W$ связно согласно
%предложению 8
%(\citeBib{Bourbaki: General Topology 1}, стр. 173).
		\end{proof}

Теорема \ref{theorem: continuity of operation} говорит
о непрерывности операции $\omega$, однако эта
теорема ничего не говорит о множествах
$W_1$, ..., $W_n$. В частности, эти множества могут быть
не связными.

Если топология на слое $A$ - дискретна,
то мы можем положить $W=\{p\}$, $W_1=\{p_1\}$, ..., $W_n=\{p_n\}$.
Возникает ощущение, что в окрестности $V$ операция не зависит от
слоя. Мы будем говорить, что операция $\omega$ локально постояна.
Однако на расслоении в целом условие постоянства может быть нарушено.
Так расслоение над окружностью со слоем группы целых чисел
может оказаться накрытием окружности $R\rightarrow S^1$
действительной прямой, определённым формулой
$p(t)=(\sin t,\cos t)$ для любого $t\in R$.

Рассмотрим альтернативную точку зрения на непрерывность операции $\omega$,
чтобы лучше понять значение непрерывности
Если мы хотим показать,
что бесконечно малые изменения операндов при движении вдоль базы
приводят к бесконечно малому изменению операции, нам надо перейти к сечениям.
Этот переход допустим,
так как операция на расслоении определена послойно.

		\begin{theorem}
		\label{theorem: operation over sections}
n-арная операция на расслоении отображает сечения в сечение.
		\end{theorem}
		\begin{proof}
Допустим $f_1$, ..., $f_n$ - сечения и отображение
	\begin{equation}
f=\omega^{\mathrm{id}}(f_1,...,f_n):M\rightarrow\mathcal{E}
	\label{eq: operation over sections}
	\end{equation}
определено равенством
	\begin{equation}
f(x)=\omega(f_1(x),...,f_n(x))
	\label{eq: operation over sections, x}
	\end{equation}
Пусть $x\in M$ и $u=f(x)$. Пусть $U$ - окрестность точки $u$ в области значений
отображения $f$.

Так как $\omega$ непрерывное отображение,
то согласно \citeBib{Bourbaki: General Topology 1}, стр. 58,
для любого значения $i$,
$1\le i\le n$ в области значений сечения $f_i$
определено открытое множество $U_i$ таким образом, что $\prod_{i=1}^nU_i$
открыто в области значений сечения $(f_1,...,f_n)$ расслоения $\mathcal{E}^n$ и
\[
\omega(\prod_{i=1}^nU_i)\subseteq U
\]

Пусть $u'\in U$.
Поскольку $f$ - отображение, существует $x'\in M$ такая, что $f(x')=u'$.
На основании равенства \eqref{eq: operation over sections, x}
существуют $u'_i\in U_i$, $p(u'_i)=x'$ такие, что
$\omega(u'_1,...,u'_n)=u'$.
%Для любого значения $i$,
%$1\le i\le n$ существует открытое множество $U_i$, содержаржащее точки
%$f_i(x')$ и $u'$.
Так как $f_i$ сечение, то существует открытое в $M$ множество $V_i$
такое, что $f_i(V_i)\subseteq U_i$
и $x\in V_i$, $x'\in V_i$. Следовательно, множество
\[
V=\cap_{i=1}^nV_i
\]
непусто, открыто в $M$ и $x\in V$, $x'\in V$.
Следовательно отображение $f$ непрерывно и является сечением.
		\end{proof}

Операция на расслоении может быть представлена диаграммой
\shorthandoff{"}
	\[
\xymatrix{
\mathcal{E}^n\ar[rr]^\omega&&\mathcal{E}\\
\times...\times\ar@{=>}@/^1pc/[rr]^{\omega^{\mathrm{id}}} &&\\
M\ars@/^2pc/[uu]^{a_1}\ars@/_2pc/[uu]_{a_n}\ar[rr]^{id}&&M\ars[uu]
}
	\]
\shorthandon{"}

		\begin{theorem}
		\label{theorem: continuous operation over sections}
$\omega^{\mathrm{id}}$ непрерывна на $\Gamma(\mathcal{E})$.
		\end{theorem}
		\begin{proof}
Рассмотрим множество $W_{K,U}$,
где $K$ - компактное подмножество пространства $M$,
$U$ - открытое подмножество пространства $\mathcal{E}$.
Множество $U$ мы можем представить в виде $V\times E$,
где $V$ - открытое множество пространства $M$, $K\subset V$.
$\omega^{-1}(V\times E)=V\times E^n$ является открытым множеством.
Следовательно,
\begin{equation}
(\omega^{\mathrm{id}})^{-1}W_{K,V\times E}=W_{K,V\times E^n}
\label{eq: continuous operation over sections}
\end{equation}
Из \eqref{eq: continuous operation over sections}
следует непрерывность $\omega^{\mathrm{id}}$.
\end{proof}

	 \begin{definition}
Пусть $A$ является $\mathcal{F}$\Hyph алгеброй
(\citeBib{Burris Sankappanavar}).
Мы можем перенести $\mathcal{F}$\Hyph алгебраическую структуру со слоя
$A$ на расслоение
$\bundle{\mathcal{A}}pAM$.
Если на $\mathcal{F}$\Hyph алгебре $A$ определена операция $\omega$
\[
a=\omega(a_1,...,a_n)
\]
то на расслоении определена операция $\omega$
\[
a(x)=\omega(a_1,...,a_n)(x)=\omega(a_1(x),...,a_n(x))
\]
Мы будем говорить, что $\bundle{}pA{}$ - это
\AddIndex{расслоенная $\mathcal{F}$\Hyph алгебра}{fibered F-algebra}.
	 \qed
	 \end{definition}

В зависимости от структуры мы будем говорить, например, о
\AddIndex{расслоенной группе}{fibered group},
\AddIndex{расслоенном кольце}{fibered ring},
\AddIndex{векторном расслоении}{vector bundle}.

Основные свойства $\mathcal{F}$\Hyph алгебры
сохраняются и для расслоенной $\mathcal{F}$\Hyph алгебры. При доказательстве
соответствующих теорем, мы можем ссылаться на это утверждение.
Однако в некоторых случаях доказательство может представлять
самостоятельный интерес, так как позволяет лучше увидеть структуру
расслоенной $\mathcal{F}$\Hyph алгебры.
Однако свойства $\mathcal{F}$\Hyph алгебры, возникшей на множестве сечений,
могут отличаться от свойств $\mathcal{F}$\Hyph алгебры в слое.
Например, умножение в слое может иметь обратный элемент.
В тоже время умножение сечений может не иметь обратного элемента.
Следовательно, расслоенное непрерывное поле порождает
кольцо на множестве сечений.
Это является преимуществом при изучении расслоенной алгебры.
Я хочу также обратить внимание на то, что операция в расслоении не определена для
элементов, принадлежащим разным слоям.

Точка $p\in\mathcal{A}$ имеет представление $(x,p_\alpha)$ в карте $U_\alpha$ и предcтавление
$(x,p_\beta)$ в карте $U_\beta$.
Допустим функции перехода $g_{\epsilon\delta}$ определяют расслоение
$\mathcal{B}$ над базой $N$.
Рассмотрим карты $V_\epsilon\in N$ и $V_\delta\in N$,
$V_\epsilon\cap V_\delta\ne\emptyset$.
Точка $q\in\mathcal{B}$ имеет представление $(y,q_\epsilon)$ в карте $V_\epsilon$ и предcтавление
$(y,q_\delta)$ в карте $V_\delta$.
Следовательно,
\[
p_\alpha=f_{\alpha\beta}(p_\beta)
\]
\[
q_\epsilon=g_{\epsilon\delta}(q_\delta)
\]
Представление соответствия при переходе от карты $U_\alpha$ к карте $U_\beta$
и от карты $V_\epsilon$ к карте $V_\delta$ изменяется согласно закону
\[
(x,y,p_\alpha,q_\epsilon)=(x,y,f_{\alpha\beta}(p_\beta),g_{\epsilon\delta}(q_\delta))
\]
Это согласуется с преобразованием
при переходе от карты $U_\alpha\times V_\epsilon$ к карте $U_\beta\times V_\delta$
в расслоении $\mathcal{A}\times\mathcal{B}$.

		\begin{theorem}
		\label{theorem: operation in two neighborhood}
Допустим функции перехода $f_{\alpha\beta}$ определяют
расслоенную $\mathcal{F}$\Hyph алгебру
$\bundle{\mathcal{A}}pAM$ над базой $M$.
Тогда функции перехода $f_{\alpha\beta}$
являются гомоморфизмами $\mathcal{F}$\Hyph алгебры $A$.
		\end{theorem}
		\begin{proof}
Пусть $U_\alpha\in M$ и $U_\beta\in M$,
$U_\alpha\cap U_\beta\ne\emptyset$ - окрестности,
в которых расслоенная $\mathcal{F}$\Hyph алгебра $\bundle{}pA{}$ тривиальна.
Пусть
	\begin{equation}
a_\beta=f_{\beta\alpha}(a_\alpha)
	\label{eq: operation in two neighborhood}
	\end{equation}
функция перехода из расслоения $\bundle{}pA{}|_{U_\alpha}$ в
расслоение $\bundle{}pA{}|_{U_\beta}$.
Пусть $\omega$ - $n$\hyph арная операция и точки $e_1$, ..., $e_n$
принадлежат слою $A_x$, $x\in U_1\cap U_2$. Положим
	\begin{equation}
e=\omega(e_1,...,e_n)
	\label{eq: operation in two neighborhood, expression}
	\end{equation}

Мы можем представить точку $e\in\bundle{}pA{}|_{U_\alpha}$ в
виде $(x,e_\alpha)$ и точку $e_i\in\bundle{}pA{}|_{U_\alpha}$ в
виде $(x,e_{i\alpha})$.
Мы можем представить точку $e\in\bundle{}pA{}|_{U_\beta}$ в
виде $(x,e_\beta)$ и точку $e_i\in\bundle{}pA{}|_{U_\beta}$ в
виде $(x,e_{i\beta})$. Согласно \eqref{eq: operation in two neighborhood}
	\begin{equation}
e_\beta=f_{\beta\alpha}(e_\alpha)
	\label{eq: operation in two neighborhood, e}
	\end{equation}
	\begin{equation}
e_{i\beta}=f_{\beta\alpha}(e_{i\alpha})
	\label{eq: operation in two neighborhood, ei}
	\end{equation}
Согласно \eqref{eq: operation in two neighborhood, expression},
операция в слое $A_x$ над окрестностью $U_\beta$ имеет вид
	\begin{equation}
e_\beta=\omega(e_{1\beta},...,e_{n\beta})
	\label{eq: operation in two neighborhood, fiber}
	\end{equation}
Подставив \eqref{eq: operation in two neighborhood, e},
\eqref{eq: operation in two neighborhood, ei} в
\eqref{eq: operation in two neighborhood, fiber} мы получим
\[
f_{\beta\alpha}(e_\alpha)=\omega(f_{\beta\alpha}(e_{1\alpha}),...,f_{\beta\alpha}(e_{n\alpha}))
\]
Это доказывает, что $f_{\beta\alpha}$ является гомоморфизмом $\mathcal{F}$\Hyph алгебры.
		\end{proof}

	\begin{definition}
	\label{definition: homomorphism of fibered F-algebras} 
Пусть $\bundle{\mathcal{A}}{p}{A}M$
и $\bundle{\mathcal{A}'}{p'}{A'}{M'}$
- две расслоенные $\mathcal{F}$\Hyph алгебры. Мы будем называть морфизм расслоений
\symb{f}0{homomorphism of fibered F-algebras}
\[
\ShowSymbol{homomorphism of fibered F-algebras}:\mathcal{A}\rightarrow\mathcal{A}'
\]
\AddIndex{гомоморфизмом расслоенных $\mathcal{F}$\Hyph алгебр}
{homomorphism of fibered F-algebras},
 если соответствующее отображение слоёв
\symb{f_x}0{fiber map}
\[
\ShowSymbol{fiber map}:A_x\rightarrow A_{x'}'
\]
является гомоморфизмом $\mathcal{F}$\Hyph алгебры $A$.
	 \qed
	 \end{definition}

	\begin{definition}
	\label{definition: isomorphism of fibered F-algebras} 
Пусть $\bundle{\mathcal{A}}{p}{A}M$
и $\bundle{\mathcal{A}'}{p'}{A'}{M'}$
- две расслоенные $\mathcal{F}$\Hyph алгебры. Мы будем называть гомоморфизм расслоенных $\mathcal{F}$\Hyph алгебр
$f$
\AddIndex{изоморфизмом расслоенных $\mathcal{F}$\Hyph алгебр}
{isomorphism of fibered F-algebras},
 если соответствующее отображение слоёв
\symb{f_x}0{fiber map}
\[
\ShowSymbol{fiber map}:A_x\rightarrow A_{x'}'
\]
является изоморфизмом $\mathcal{F}$\Hyph алгебры $A$.
	 \qed
	 \end{definition}

	\begin{definition}
Пусть $\bundle{\mathcal{A}}pAM$ -
расслоенная $\mathcal{F}$\Hyph алгебра и $A'$ - $\mathcal{F}$\Hyph подалгебра
$\mathcal{F}$\Hyph алгебры $A$.
Расслоенная $\mathcal{F}$\Hyph алгебра
$\bundle{\mathcal{A}'}p{A'}M$
является \AddIndex{расслоенной $\mathcal{F}$\Hyph подалгеброй}{fibered F-subalgebra}
расслоенной $\mathcal{F}$\Hyph алгебры
$\bundle{}pA{}$,
если гомоморфизм расслоенных $\mathcal{F}$\Hyph алгебр
$\mathcal{A}'\rightarrow\mathcal{A}$
является вложением слоёв.
	 \qed
	 \end{definition}

Важным обстоятельством в этом определении является гомоморфизм расслоенных $\mathcal{F}$\Hyph алгебр.
Если мы просто ограничимся фактом существования $\mathcal{F}$\Hyph подалгебры в каждом слое,
то мы можем разрушить непрерывность.

Мы определили операцию на базе приведенного декартова произведения расслоений.
Если мы определим операцию на базе декартова произведения расслоений,
то операция будет определена для любых элементов расслоения. Однако,
если $p(a_i)=p(b_i)$, $i=1$, ..., $n$, то $p(\omega(a_1,...,a_n))=p(\omega(b_1,...,b_n))$.
Следовательно, операция определена между слоями и посредством проекции
переносится на базу. Эта конструкция не отличается от факторизации $\mathcal{F}$\Hyph алгебры
и не создаёт новый элемент в теории расслоений. В то же время эта конструкция
довольно проблематична с точки зрения перехода между различными картами
расслоения и возможности определения операции над сечениями. 

			\section{Представление расслоенной \texorpdfstring{$\mathcal{F}$}{F}\Hyph алгебры}
			\label{section: Representation of Fibered F-Algebra}

	\begin{definition}
	\label{definition: nonsingular transformation, bundle} 
Мы будем называть морфизм расслоений
\[
t:\mathcal{E}\rightarrow\mathcal{E}
\]
\AddIndex{преобразованием расслоения}
{transformation of bundle},
если соответствующее отображение слоёв
\[
t_x:E_x\rightarrow E_x
\]
является преобразованием слоя.
	 \qed
	 \end{definition}

		\begin{theorem}
		\label{theorem: continuity of transformation}
Пусть $U$ - открытое множество базы $M$,
на котором существует тривиализация расслоения $\bundle{}pE{}$.
Пусть $t$ - преобразование расслоения $\bundle{}pE{}$.
Пусть $x\in M$ и $p'=t_x(p)$ в слое $E_x$.
Тогда для открытого множества $V\subseteq M$,
$x\in V$ и для открытого множества $W'\subseteq E$,
$p'\in W'$
существует открытое множество $W\subseteq E$,
такое, что если $x_1\in V$, $p_1\in W$,
то $p'_1=t_{x_1}(p_1)\in W$.
		\end{theorem}
		\begin{proof}
Согласно \citeBib{Bourbaki: General Topology 1}, стр. 58,
множества вида $V\times W$, где $V$ принадлежит базису
топологии пространства $U$ и $W$ принадлежит базису топологии пространства $E$,
образуют базис топологии пространства $\mathcal{E}$. 

Так как отображение $t$ непрерывно, то для открытого множества
$V\times W'$ существует открытое множество $V\times W$ такое,
что $t( V\times W)\subseteq V\times W'$. Это и есть содержание теоремы.
		\end{proof}

		\begin{theorem}
		%\label{theorem: continuity of operation}
Преобразованием расслоения $\bundle{}pE{}$
отображает сечение в сечение.
		\end{theorem}
		\begin{proof}
Образ сечения $s$ при преобразовании $t$
определён из коммутативности диаграммы
	\[
\xymatrix{
\mathcal{E}\ar[rr]^t&&\mathcal{E}\\
&M\ars[ul]^s\ars[ur]_{s'}&
}
	\]
Непрерывность отображения $s'$
следует из теоремы
\ref{theorem: continuity of transformation}.
		\end{proof}

	 \begin{definition}
	\label{definition: Tstar transformation of bundle} 
Преобразование расслоения называется
\AddIndex{левосторонним преобразованием}{left-side transformation of bundle}
или
\AddIndex{\Ts преобразованием расслоения}{Tstar transformation of bundle},
если оно действует слева
\[
u'=t u
\]
Мы будем обозначать
\symb{{}^\star \mathcal{E}}1
{set of Tstar nonsingular transformations of bundle} или
\symb{{}^\star \bundle{}pE{}}1
{set of Tstar nonsingular transformations of bundle, projection}
множество невырожденных \Ts преобразований расслоения
$\bundle{}pE{}$.
	 \qed
	 \end{definition}

	 \begin{definition}
Преобразование называется
\AddIndex{правосторонним преобразованием}
{right-side transformation of bundle}
или
\AddIndex{\sT преобразованием расслоения}{starT transformation of bundle},
если оно действует справа
\[
u'= ut
\]
Мы будем обозначать
\symb{\mathcal{E}^\star}1{set of starT nonsingular transformations of bundle} или
\symb{\bundle{}pE{}^\star}1{set of starT nonsingular transformations of bundle, projection}
множество \sT невырожденных преобразований расслоения
$\bundle{}pA{}$.
	 \qed
	 \end{definition}

Мы будем обозначать
\symb{e}1{identical transformation of bundle}
тождественное преобразование расслоения.

Так как \Ts преобразованием расслоения определено послойно, то множество ${}^\star \bundle{}pE{}$
является расслоением, изоморфным расслоению $\bundle{}p{{}^\star E}{}$.

		\begin{definition}
		\label{definition: Tstar representation of fibered F-algebra} 
Пусть на множестве ${}^\star \bundle{}pA{}$
определена структура расслоенной $\mathcal{F}$\Hyph алгебры
(\citeBib{Burris Sankappanavar}).
Пусть $\bundle{}pB{}$ является расслоенной $\mathcal{F}$\Hyph алгеброй.
Мы будем называть гомоморфизм расслоенных $\mathcal{F}$\Hyph алгебр
	\begin{equation}
f:\bundle{}pB{}\rightarrow {}^\star \bundle{}pA{}
	\label{eq: Tstar representation of fibered F-algebra}
	\end{equation}
\AddIndex{левосторонним представлением}
{left-side representation of fibered F-algebra} или
\AddIndex{\Ts представлением расслоенной $\mathcal{F}$\Hyph алгебры $\bundle{}pB{}$}
{Tstar representation of fibered F-algebra}.
		\qed
		\end{definition}

		\begin{definition}
		\label{definition: starT representation of fibered F-algebra} 
Пусть на множестве $\bundle{}pA{}^\star$
определена структура расслоенной $\mathcal{F}$\Hyph алгебры
(\citeBib{Burris Sankappanavar}).
Пусть $\bundle{}pB{}$ является расслоенной $\mathcal{F}$\Hyph алгеброй.
Мы будем называть гомоморфизм расслоенных $\mathcal{F}$\Hyph алгебр
	\[
f:\bundle{}pB{}\rightarrow \bundle{}pA{}^\star
	\]
\AddIndex{правосторонним представлением}
{right-side representation of fibered F-algebra} или
\AddIndex{\sT представлением расслоенной $\mathcal{F}$\Hyph алгебры $\bundle{}pB{}$}
{starT representation of fibered F-algebra}.
		\qed
		\end{definition}

Мы распространим на теорию расслоенных представлений соглашение,
описанное в замечании
\xRef{0701.238}{remark: left and right matrix notation}.
Мы можем записать принцип двойственности в следующей форме

		\begin{theorem}[принцип двойственности]
		\label{theorem: duality principle, fibered F-algebra representation}
Любое утверждение, справедливое для
\Ts представления расслоенной $\mathcal{F}$\Hyph алгебры $\bundle{}pA{}$,
будет справедливо для \sT представления расслоенной $\mathcal{F}$\Hyph алгебры $\bundle{}pA{}$.
		\end{theorem}

Существует два способа определить \Ts представление $\mathcal{F}$\Hyph алгебры $B$ в расслоении
$\bundle{}pA{}$. Мы можем определить определить \Ts представление в слое,
либо определить \Ts представление на множестве $\Gamma(\bundle{}pA{})$.
В первом случае представление определяет одно и то же преобразование во
всех слоях. Во втором случае картина менее ограничена, однако она не даёт полной
картины разнообразия представлений в расслоении. Когда мы рассматриваем представление
расслоенной $\mathcal{F}$\Hyph алгебры, мы сразу оговариваем, что преобразования в разных слоях
независимы. Требование непрерывной зависимости преобразования
от слоя накладывает дополнительные ограничения на \Ts представление расслоенной $\mathcal{F}$\Hyph алгебры.
В то же время это ограничение позволяет изучать представления расслоенных $\mathcal{F}$\Hyph алгебр,
когда в слое определена $\mathcal{F}$\Hyph алгебра, параметры которой
(например, структурные константы группы Ли) непрерывно зависят от слоя.

		\begin{remark}
		\label{remark: reduce details on the diagram, fibered F-algebra}
На языке диаграмм определение
\ref{definition: Tstar representation of fibered F-algebra}
означает следующее.
\shorthandoff{"}
	\[
\xymatrix{
\mathcal{E}&\mathcal{E}'\arp[dr]_{p'}\ar[rr]^\varphi="C2"
& & \mathcal{E}'\arp[dl]^{p'}\\
M\ars[u]^\alpha="C1"\ar[rr]^F& & M'\\
\ar @{=>}@/_1pc/ "C1";"C2"
}
	\]
\shorthandon{"}%
Отображение $F$ - инъекция. Так как мы ожидаем, что представление расслоенной
$\mathcal{F}$\Hyph алгебры действует в каждом слое, то мы видим, что отображение $F$ - биекция.
Не нарушая общности, мы можем положить, что $M=M'$ и отображение $F$ - тождественное
отображение. Мы будем говорить, что задано представление расслоенной $\mathcal{F}$\Hyph алгебры
$\bundle{}pB{}$ в расслоении $\bundle{}pA{}$ над множеством $M$.
Поскольку база расслоения известна, то, чтобы не перегружать диаграмму деталями, мы будем
описывать представление с помощью диаграммы
\shorthandoff{"}
	\[
\xymatrix{
\mathcal{E}&\mathcal{E}'\ar[rr]^\varphi="C2"
& & \mathcal{E}'\\
M\ars[u]^\alpha="C1"\\
\ar @{=>}@/_1pc/ "C1";"C2"
}
	\]
\shorthandon{"}%
		\qed
		\end{remark}

	 \begin{definition}
	 \label{definition: effective representation of fibered F-algebra}
Мы будем называть \Ts представление расслоенной $\mathcal{F}$\Hyph алгебры $\bundle{}pB{}$
\AddIndex{эффективным}{effective representation of fibered F-algebra},
если отображение \eqref{eq: Tstar representation of fibered F-algebra} -
изоморфизм расслоенной $\mathcal{F}$\Hyph алгебры $\bundle{}pB{}$ в ${}^\star \bundle{}pA{}$.
	 \qed
	 \end{definition}

		\begin{remark}
		\label{remark: notation for effective representation of fibered F-algebra}
Если \Ts представление расслоенной $\mathcal{F}$\Hyph алгебры эффективно, мы можем отождествлять
элемент расслоенной $\mathcal{F}$\Hyph алгебры с его образом и записывать \Ts преобразование,
порождённое элементом $a\in A$,
в форме
\[v'=av\]
Если \sT представление расслоенной $\mathcal{F}$\Hyph алгебры эффективно, мы можем отождествлять
элемент $\mathcal{F}$\Hyph алгебры с его образом и записывать \sT преобразование,
порождённое элементом $a\in A$,
в форме
\[v'=va\]
		\qed
		\end{remark}

	 \begin{definition}
	 \label{definition: transitive representation of fibered F-algebra}
Мы будем называть \Ts представление расслоенной $\mathcal{F}$\Hyph алгебры
\AddIndex{транзитивным}{transitive representation of fibered F-algebra},
если для любых $a, b \in V$ существует такое $g$, что
\[a=f(g)b\]
Мы будем называть \Ts представление расслоенной $\mathcal{F}$\Hyph алгебры
\AddIndex{однотранзитивным}{single transitive representation of fibered F-algebra},
если оно транзитивно и эффективно.
	 \qed
	 \end{definition}

		\begin{theorem}	%однотранзитивное
\Ts представление однотранзитивно тогда и только тогда, когда для любых $a, b \in M$
существует одно и только одно $g\in A$ такое, что $a=f(g)b$
		\end{theorem}
		\begin{proof}
Следствие определений \ref{definition: effective representation of fibered F-algebra}
и \ref{definition: transitive representation of fibered F-algebra}.
		\end{proof}


==> Fibered.Group.Russian.tex <==
%auto-ignore
\def\texFiberedGroup{}

			\section{Представление расслоенной группы}
			\label{section: Representation of fibered group}

	\begin{definition}
	\label{definition: homomorphism of fibered groups} 
Пусть $\bundle{\mathcal{G}}{p}GM$
и $\bundle{\mathcal{G}'}{p'}{G'}{M'}$
- две расслоенные группы. Мы будем называть морфизм расслоений
\[
f:\mathcal{G}\rightarrow\mathcal{G}'
\]
\AddIndex{гомоморфизмом расслоенных групп}{homomorphism of fibered groups},
 если соответствующее отображение слоёв
\[
f_x:G_x\rightarrow G_{x'}'
\]
является гомоморфизмом групп.
	 \qed
	 \end{definition}

	\begin{definition}
	\label{definition: antihomomorphism of fibered groups} 
Пусть $\bundle{\mathcal{G}}{p}GM$
и $\bundle{\mathcal{G}'}{p'}{G'}{M'}$
- две расслоенные группы. Мы будем называть морфизм расслоений
\[
f:\mathcal{G}\rightarrow\mathcal{G}'
\]
\AddIndex{антигомоморфизмом расслоенных групп}{antihomomorphism of fibered groups},
 если соответствующее отображение слоёв
\[
f_x:G_x\rightarrow G_{x'}'
\]
является антигомоморфизмом групп.
	 \qed
	 \end{definition}

		\begin{definition}
		\label{definition: Tstar representation of fibered group} 
Пусть $\bundle{}pG{}$ - расслоенная группа.
Мы будем называть отображение
	\begin{equation}
f:\bundle{}pG{}\rightarrow {}^\star \bundle{}pA{}
	\label{eq: Tstar representation of fibered group}
	\end{equation}
\AddIndex{\Ts представлением расслоенной группы}
{Tstar representation of fibered group}
$\bundle{}pG{}$ в расслоении $\bundle{}pA{}$,
если отображение $f$ удовлетворяет условиям
	\begin{equation}
f(ab)\mu=f(a)(f(b)\mu)
	\label{eq: Tstar product of bundle transformations}
	\end{equation}
	\begin{equation}
f(\epsilon)=e
	\label{eq: Tstar identical transformation of bundle}
	\end{equation}
		\qed
		\end{definition}

		\begin{definition}
		\label{definition: starT representation of fibered group} 
Пусть $\bundle{}pG{}$ - расслоенная группа.
Мы будем называть отображение
	\begin{equation}
f:\bundle{}pG{}\rightarrow\bundle{}pA{}^\star
	\label{eq: starT representation of fibered group}
	\end{equation}
\AddIndex{\sT представлением расслоенной группы}
{starT representation of fibered group}
$\bundle{}pG{}$ в расслоении $\bundle{}pA{}$,
если отображение $f$ удовлетворяет условиям
	\begin{equation}
\mu f(ab)=(\mu f(a))f(b)
	\label{eq: starT product of bundle transformations}
	\end{equation}
	\begin{equation}
f(\epsilon)=e
	\label{eq: starT identical transformation of bundle}
	\end{equation}
		\qed
		\end{definition}

			\begin{theorem}
			\label{theorem: inverse bundle transformation}
Для любого $a\in \bundle{}pG{}$
	\begin{equation}
	\label{eq: inverse bundle transformation}
f(a^{-1})=f(a)^{-1}
	\end{equation}
		\end{theorem}
		\begin{proof}
На основании \eqref{eq: Tstar product of bundle transformations}
и \eqref{eq: Tstar identical transformation of bundle},
мы можем записать
\[
\mu=e \mu=f(aa^{-1})\mu
=f(a)(f(a^{-1})\mu)
\]
Это завершает доказательство.
		\end{proof}

		\begin{theorem}
		\label{theorem: Tstar covariant representation of fibered group}
Пусть ${}^\star \bundle{}pA{}$ -
расслоенная группа относительно умножения
	\begin{equation}
(t_1t_2)\mu=t_1(t_2\mu)
	\label{eq: Tstar covariant product of bundle transformations}
	\end{equation}
и $e$ - единица расслоенной группы ${}^\star \bundle{}pA{}$.
Если отображение
\eqref{eq: Tstar representation of fibered group}
является гомоморфизмом расслоенных групп
	\begin{equation}
f(ab)=f(a)f(b)
	\label{eq: Tstar covariant representation of bundle group}
	\end{equation}
то это отображение является представлением расслоенной группы $\bundle{}pG{}$,
которое мы будем называть
\AddIndex{ковариантным \Ts представлением расслоенной группы}
{Tstar covariant representation of fibered group}.
		\end{theorem}
		\begin{proof}
Так как $f$ - гомоморфизм расслоенных групп,
то $f(\epsilon)=e$.

Согласно
\eqref{eq: Tstar covariant product of bundle transformations}
и \eqref{eq: Tstar covariant representation of bundle group}
\[
f(ab)\mu=(f(a)f(b))\mu
=f(a)(f(b)\mu)
\]

Согласно определению \ref{definition: Tstar representation of fibered group}
$f$ является представлением расслоенной группы.
		\end{proof}

Ковариантное \Ts представление расслоенной группы на расслоении может быть представлено диаграммой
\shorthandoff{"}
	\[
\xymatrix{
&&&&&\mathcal{E}\ar[dd]^{f(ab)}="f(ab)"\ar[lld]_{f(a)}="f(a)"\\
&&&\mathcal{E}\ar[drr]_{f(b)}="f(b)"&&\\
\mathcal{G}^2\ar[rr]&&\mathcal{G}&&&\mathcal{E}\\
\odot\ar@{=>}@/^1pc/[rr] &&&&&\\
M\ars@/^2pc/[uu]^a="a"\ars@/_2pc/[uu]_b="b"\ar[rr]^{id}&&
M\ars[uu]_{ab}="ab"&&&
\ar @{=>}@/_4pc/ "ab";"f(ab)"
\ar @{=>}@/^4pc/ "a";"f(a)"
\ar @{=>}@/^3pc/ "b";"f(b)"
}
	\]
\shorthandon{"}

		\begin{theorem}
		\label{theorem: Tstar contravariant representation of fibered group}
Пусть ${}^\star \bundle{}pA{}$ - расслоенная группа относительно умножения
	\begin{equation}
(t_2t_1)\mu=t_1(t_2\mu)
	\label{eq: Tstar contravariant product of bundle transformations}
	\end{equation}
и $e$ - единица расслоенной группы ${}^\star \bundle{}pA{}$.
Если отображение
\eqref{eq: Tstar representation of fibered group}
является антигомоморфизмом расслоенных групп
	\begin{equation}
f(ba)=f(a)f(b)
	\label{eq: Tstar contravariant representation of bundle group}
	\end{equation}
то это отображение является представлением расслоенной группы $\bundle{}pG{}$,
которое мы будем называть
\AddIndex{контравариантным \Ts представлением расслоенной группы}
{Tstar contravariant representation of fibered group}.
		\end{theorem}
		\begin{proof}
Так как $f$ - антигомоморфизм расслоенных групп,
то $f(\epsilon)=e$.

Согласно
\eqref{eq: Tstar contravariant product of bundle transformations}
и \eqref{eq: Tstar contravariant representation of bundle group}
\[
f(ab)\mu=(f(b)f(a))\mu
=f(a)(f(b)\mu)
\]

Согласно определению \ref{definition: Tstar representation of fibered group}
$f$ является представлением расслоенной группы.
		\end{proof}

	\begin{example}
Групповая операция на расслоении групп
определяет два различных представления на расслоении групп:
\AddIndex{\Ts сдвиг на расслоении групп}
{Tstar shift, fibered group},
который мы определяем равенством
\symb{a\star b}0{Tstar shift, fibered group}
	\begin{equation}
b'=\ShowSymbol{Tstar shift, fibered group}=ab
	\label{eq: Tstar shift, fibered group}
	\end{equation}
и \AddIndex{\sT сдвиг на расслоении групп}
{starT shift, fibered group},
который мы определяем равенством
\symb{b\star a}0{starT shift, fibered group}
	\begin{equation}
b'=\ShowSymbol{starT shift, fibered group}=ba
	\label{eq: starT shift, fibered group}
	\end{equation}
	 \qed
	 \end{example}

	\begin{example}
Пусть $\bundle{}p{GL}{}$ расслоение над осью вещественных чисел. Задавшись матрицей
$A$, мы можем определить сечение $a(t)=exp(tA)$, и это сечение будет порождать
соответствующий \Ts сдвиг.
	 \end{example}

	 \begin{definition}
Пусть $f$ - представлением расслоенной группы
$\bundle{}pG{}$ в расслоении $\bundle{}pA{}$.
Для любого сечения $u$ расслоения $\bundle{}pA{}$ мы определим его
\AddIndex{орбиту представления расслоенной группы}
{orbit of representation of fibered group}
как множество
\symb{\mathcal{O}(u,g\in\Gamma(\bundle{}pG{}),f(g)u)}
0{orbit of representation of fibered group}
\[
\ShowSymbol{orbit of representation of fibered group}
=\{v=f(g)u:g\in\Gamma(\bundle{}pG{})\}
\]
	 \qed
	 \end{definition}

$u\in\mathcal{O}(u,g\in\Gamma(\bundle{}pG{}),f(g)u)$,
так как $f(\epsilon)=e$.

		\begin{theorem}
		\label{theorem: proper definition of orbit, fibered group}
Если
	\begin{equation}
	\label{eq: orbit, fibered group, proposition}
v\in\mathcal{O}(u,g\in\Gamma(\bundle{}pG{}),f(g)u)
	\end{equation}
то
\[
\mathcal{O}(u,g\in\Gamma(\bundle{}pG{}),f(g)u)
=\mathcal{O}(v,g\in\Gamma(\bundle{}pG{}),f(g)v)
\]
		\end{theorem}
		\begin{proof}
Из \eqref{eq: orbit, fibered group, proposition} следует
существование $\mu\in\Gamma(\bundle{}pG{})$ такого, что
	\begin{equation}
v=f(\mu)u
	\label{eq: orbit, fibered group, 1}
	\end{equation}
Если $\delta\in\mathcal{O}(v,g\in\Gamma(\bundle{}pG{}),f(g)v)$, то
существует $\nu\in\Gamma(\bundle{}pG{})$ такой, что
	\begin{equation}
\delta=f(\nu)v
	\label{eq: orbit, fibered group, 2}
	\end{equation}
Подставив \eqref{eq: orbit, fibered group, 1} в \eqref{eq: orbit, fibered group, 2}, мы получим
	\begin{equation}
\delta=f(\nu)f(\mu)u
	\label{eq: orbit, fibered group, 3}
	\end{equation}
На основании \eqref{eq: Tstar product of bundle transformations}
из \eqref{eq: orbit, fibered group, 3} следует,
что $\delta\in\mathcal{O}(u,g\in\Gamma(\bundle{}pG{}),f(g)u)$.
Таким образом,
\[
\mathcal{O}(v,g\in\Gamma(\bundle{}pG{}),f(g)v)
\subseteq\mathcal{O}(u,g\in\Gamma(\bundle{}pG{}),f(g)u)
\]

На основании \eqref{eq: inverse bundle transformation} из
\eqref{eq: orbit, fibered group, 1} следует,
что
	\begin{equation}
u=f(\mu)^{-1}v=f(\mu^{-1})v
	\label{eq: orbit, fibered group, 4}
	\end{equation}
Равенство \eqref{eq: orbit, fibered group, 4} означает, что
$u\in\mathcal{O}(v,g\in\Gamma(\bundle{}pG{}),f(g)v)$ и, следовательно,
\[
\mathcal{O}(u,g\in\Gamma(\bundle{}pG{}),f(g)u)
\subseteq\mathcal{O}(v,g\in\Gamma(\bundle{}pG{}),f(g)v)
\]
Это завершает доказательство.
		\end{proof}

Допустим, что определено представление группы $G$ на расслоении $$\bundle{\mathcal{E}}pA{M}$$
Если мы говорим, что представление транзитивно, то это означает, что орбита точки
- это всё многообразие $\mathcal{E}$. В случае представления
расслоенной группы $\bundle{}pG{}$ орбита точки является слоем, содержащим эту точку.

		 \begin{theorem}
		 \label{theorem: direct product of representations of fibered group}
Если определены представление $f_1$
расслоенной группы $\bundle{}pG{}$ в расслоении $\bundle{}p{A_1}{}$
и представление $f_2$ расслоенной группы $\bundle{}pG{}$
в расслоении $\bundle{}p{A_2}{}$,
то мы можем определить
\AddIndex{прямое произведение представлений
$f_1$ и $f_2$ расслоенной группы}
{direct product of representations of fibered group} $\bundle{}pG{}$
	\begin{align*}
f&=f_1\otimes f_2:
\bundle{}pG{}\rightarrow \bundle{}p{A_1}{}\otimes \bundle{}p{A2}{}\\
f(g)&=(f_1(g),f_2(g))
	\end{align*}
		\end{theorem}
		\begin{proof}
Чтобы показать, что $f$ является представлением,
достаточно показать, что $f$ удовлетворяет определению
\ref{definition: Tstar representation of fibered group}.
\[f(e)=(f_1(e),f_2(e))
=(e_1,e_2)=e\]
	\begin{align*}
f(ab)u&=(f_1(ab)u_1,f_2(ab)u_2)\\
&=(f_1(a)(f_1(b)u_1),
f_2(a)(f_2(b)u_2))\\
&=f(a)(f_1(b)u_1,f_2(b)u_2)\\
&=f(a)(f(b)u)
	\end{align*}
		\end{proof}

			\section{Однотранзитивное представление}

	 \begin{definition}
	 \label{definition: kernel of inefficiency of representation of fibered group}
Мы будем называть
\AddIndex{ядром неэффективности представления расслоенной группы}
{kernel of inefficiency of representation of fibered group} $\bundle{}pG{}$
множество \[K_f=\{g\in\Gamma(\bundle{}pG{}):f(g)=e\}\]
Если $K_f=\{e\}$, мы будем называть представление расслоенной группы $G$
\AddIndex{эффективным}{effective representation of fibered group}.
	 \qed
	 \end{definition}

		\begin{theorem}
		\label{theorem: kernel of inefficiency, representation of fibered group}
Ядро неэффективности - это подгруппа расслоенной группы $G$.
		\end{theorem}
		\begin{proof}
Доказательство не зависит от типа представления, которое мы используем:
ковариантное или
контравариантное. Пусть $f$ - ковариантное представление и
$f(a_1)=\delta$ и $f(a_2)=\delta$. Тогда
\[f(a_1a_2)=f(a_1)f(a_2)=\delta\]
\[f(a^{-1})=f^{-1}(a)=\delta\]
		\end{proof}

%Если действие не эффективно, мы можем перейти к эффективному
%заменив группой $G_1=G|K_f$,
%пользуясь факторизацией по ядру неэффективности.
%Это означает, что мы можем изучать только эффективное действие.

		\begin{theorem}	%однотранзитивное
Представление однотранзитивно тогда и только тогда, когда для любых $a, b \in\Gamma(\bundle{}pA{})$
существует одно и только одно $g\in\bundle{}pG{}$ такое, что $a=f(g)b$
		\end{theorem}
		\begin{proof}
Утверждение является следствием определений
\ref{definition: effective representation of fibered F-algebra} и
\ref{definition: kernel of inefficiency of representation of fibered group} и
теоремы \ref{theorem: kernel of inefficiency, representation of fibered group}.
		\end{proof}

	 \begin{definition}
Мы будем называть расслоение $\bundle{}pA{}$
\AddIndex{однородным расслоением расслоенной группы}
{homogeneous bundle of fibered group} $\bundle{}pG{}$,
если мы имеем однотранзитивное представление расслоенной группы $\bundle{}pG{}$ на $\bundle{}pA{}$.
	 \qed
	 \end{definition}

		\begin{theorem}	%
		\label{theorem: single transitive representation of fibered group}
Если мы определим однотранзитивное \Ts представление $f$ расслоенной группы $\bundle{}pG{}$
в расслоении $\bundle{}pA{}$,
то мы можем однозначно определить координаты на $\bundle{}pA{}$,
пользуясь координатами на расслоенной группе $\bundle{}pG{}$.

Если $f$ - ковариантное однотранзитивное представление,
то $f(a)$ эквивалентно левому сдвигу $a\star$ на расслоенной группе $\bundle{}pG{}$.
Если $f$ = контравариантное однотранзитивное представление,
то $f(a)$ эквивалентно правому сдвигу $\star a$ на расслоенной группе $\bundle{}pG{}$.
		\end{theorem}
		\begin{proof}
Представление расслоенной группы $\bundle{}pG{}$ в расслоении $\bundle{}pA{}$ однотранзитивно
тогда и только тогда, когда однотранзитивно представление группы $G$ на слое $A_x$ для любого $x$.
Допустим представление $f$ расслоенной группы $\bundle{}pG{}$ - 
ковариантное однотранзитивное представление.
Пусть $u$, $v$ - сечения расслоения $\bundle{}pA{}$.
Выбрав произвольный $x$, мы найдём
согласно теореме
\xRef{0701.238}{theorem: single transitive representation of group}
единственный элемент $g_x\in G$ такой, что
\[
u(x)=f(g_x)v(x)=g_xv(x)
\]
Таким образом, отображение $x\rightarrow g_x$ является искомым сечением расслоения групп $\bundle{}pG{}$.

Аналогично доказывается утверждение для контравариантного однотранзитивного представления.

Чтобы доказать первое утверждение, мы должны выделить
карту на многообразии $M$, где оба расслоения тривиальны. В этом случае, мы можем
представить координаты точки $u\in\bundle{}pA{}$ как упорядоченную пару координат
$(x,y)$, где $x$ - координаты проекции на многообразие $M$, и $y$ - координаты
точки в слое. Мы можем
представить координаты точки $a\in\bundle{}pG{}$ как упорядоченную пару координат
$(x,g)$, где $x$ - координаты проекции на многообразие $M$, и $g$ - координаты
точки в группе. Соответственно, координаты сечения расслоения $\bundle{}pA{}$ -
это отображение $y:M\rightarrow A$, и координаты сечения расслоения $\bundle{}pG{}$ -
это отображение $y:M\rightarrow G$.

Мы выберем сечение $v\in\Gamma(\bundle{}pA{})$
и определим координаты сечения $w\in\Gamma(\bundle{}pA{})$
как координаты $a\in\bundle{}pG{}$ такого, что $w=f(a) v$.
Координаты, определённые таким образом, однозначны
с точностью до выбора начального сечения $v\in\Gamma(\bundle{}pA{})$,
так как действие эффективно.
		\end{proof}

		\begin{remark}
Мы будем записывать \Ts ковариантное эффективное
представление расслоенной группы $\bundle{}pG{}$ в форме
\[v'=a\star v=av\]
Орбита этого представления имеет вид
\symb{\bundle{}pG{}v}0{orbit of effective Tstar covariant representation of fibered group}
\[
\ShowSymbol{orbit of effective Tstar covariant representation of fibered group}
=\bundle{}pG{}\star v
\]
		\qed
		\end{remark}

		\begin{remark}
Мы будем записывать \sT ковариантное эффективное
представление расслоенной группы $\bundle{}pG{}$ в форме
\[v'=v\star a=va\]
Орбита этого представления имеет вид
\symb{v\bundle{}pG{}}0{orbit of effective starT covariant representation of fibered group}
\[
\ShowSymbol{orbit of effective starT covariant representation of fibered group}
=v\star\bundle{}pG{}
\]
		\qed
		\end{remark}

		\begin{theorem}	%
		\label{theorem: shifts on fibered group commuting}
Левый и правый сдвиги на расслоенной группе $\bundle{}pG{}$ перестановочны.
		\end{theorem}
		\begin{proof}
Это следствие ассоциативности расслоенной группы $\bundle{}pG{}$
\[(a\star \star b)c = a(cb)=(ac)b=(\star b\ a\star)c\]
		\end{proof}

		\begin{theorem}	%
		\label{theorem: two representations of fibered group}
Если мы определили однотранзитивное ковариантное \Ts представление $f$
расслоенной группы $\bundle{}pG{}$ на расслоении $\bundle{}pA{}$,
то мы можем однозначно определить однотранзитивное ковариантное \sT представление $h$
расслоенной группы $\bundle{}pG{}$ на расслоении $\bundle{}pA{}$
такое, что диаграмма
\shorthandoff{"}
	\[
\xymatrix{
\mathcal{G}&&\mathcal{E}\ar[rr]^{h(a)}="Ct2"\ar[dd]^{f(b)}="Cl2"
& & \mathcal{E}\ar[dd]^{f(b)}="Cr2"\\
&&&&\\
M\ars@/^2pc/[uu]^b="Cl1"\ars@/_2pc/[uu]_a="Cr1"&&\mathcal{E}\ar[rr]_{h(a)}="Cb2"
& & \mathcal{E}\\
\ar @{=>}@/_1pc/ "Cr1";"Ct2"
\ar @{=>}@/_2pc/ "Cr1";"Cb2"
\ar @{=>}@/_1pc/ "Cl1";"Cl2"
\ar @{=>}@/_1.5pc/ "Cl1";"Cr2"
}
	\]
\shorthandon{"}%
коммутативна для любых $a$, $b\in \Gamma(\bundle{}pG{})$.
		\end{theorem}
		\begin{proof}
Предположим, что $f$ - однотранзитивное ковариантное \Ts представление.
В каждом слое $A_x$ представление $f$ определяет однотранзитивное ковариантное \Ts представление
$f_x$ группы $G$. Согласно теореме
\xRef{0701.238}{theorem: two representations of group}
в слое $A_x$ однозначно определено однотранзитивное ковариантное \sT представление
$h_x$, перестановочное с представлением $f_x$.
Для сечения $a\in\Gamma(\bundle{}pG{})$ определено сечение
\[
h(a):x\rightarrow h_x(a)
\] 
Отображение $h$ является гомоморфизмом расслоенных групп.
		\end{proof}

Мы будем называть представления $f$ и $h$
\AddIndex{парными преставлениями расслоенной группы}{twin representations of fibered group}
$\bundle{}pG{}$.

==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index{texLinearMap}%1%1
   {$1$-\drc форма}%
   {1-drc form, vector spaces}%
\SetIndexSpace%
\Index{texPolymodule}%2%66
   {$(2)$\hyph векторное пространство}%
   {(2)-vector space}%
\Index{texBundleRelation}%2%122
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index{texBiring}%A%2
   {$(^{\gi a}_{\gi b})$\hyph \CR квазидетерминант}%
   {a b cr-quasideterminant}%
\Index{texBiring}%A%34
   {$(^{\gi a}_{\gi b})$\hyph \RC квазидетерминант}%
   {a b RC-quasideterminant}%
\Index{texCalculus}%A%67
   {$A$\Hyph значная функция}%
   {A valued function}%
\SetIndexSpace%
\Index{texBiring}%C%3
   {\subs строка матрицы}%
   {c row}%
\Index{texVectorSpace}%C%5
   {\CR матричная группа}%
   {cr-matrix group}%
\Index{texBiring}%C%6
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index{texBiring}%C%7
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Index{texBiring}%C%8
   {\CR степень}%
   {cr power}%
\Index{texVectorSpace}%C%9
   {\crd векторное пространство}%
   {crd vector space}%
\Index{texBiring}%C%10
   {$c$\hyph строка матрицы}%
   {c-row}%
\SetIndexSpace%
\Index{texVectorSpace}%D%11
   {\dcr базис векторного пространства \subs строк}%
   {dcr basis, c rows vector space}%
\Index{texVectorSpace}%D%12
   {\dcr вектор}%
   {dcr vector}%
\Index{texVectorSpace}%D%13
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index{texVectorSpace}%D%14
   {\dcr векторное пространство \subs строк}%
   {subs rows dcr vector space}%
\Index{texVectorSpace}%D%15
   {\drc  линейно зависимые векторы}%
   {linearly dependent, vector space}%
\Index{texVectorSpace}%D%55
   {\drc автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index{texVectorSpace}%D%17
   {\drc базис}%
   {}%
\SubIndex{texVectorSpace}%4%
   {в векторном пространстве}%
   {drc basis, vector space}%
\SubIndex{texVectorSpace}%5%
   {в векторном пространстве \sups строк}%
   {drc basis, r rows vector space}%
\Index{texVectorSpace}%D%18
   {\drc вектор}%
   {drc vector}%
\Index{texVectorSpace}%D%19
   {\drc векторное пространство}%
   {drc vector space}%
\Index{texVectorSpace}%D%20
   {\drc векторное пространство \sups строк}%
   {sups rows drc vector space}%
\Index{texCalculus}%D%46
   {\drc вектор\hyph функция}%
   {drc vector function}%
\Index{texVectorSpace}%D%83
   {\drc изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index{texVectorSpace}%D%87
   {\drc координатное векторное пространство}%
   {drc coordinate vector space}%
\Index{texVectorSpace}%D%23
   {\drc линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\Index{texReferenceFrame}%D%24
   {\drc линейно независимыe векторы}%
   {linearly independent vector fields}%
\Index{texVectorSpace}%D%114
   {\drc линейно независимые векторы}%
   {linearly independent, vector space}%
\Index{texDrcMorphism}%D%25
   {\drc линейное отображение векторных пространств}%
   {drc linear map of vector spaces}%
\Index{texVectorSpace}%D%27
   {$D\star$\hyph векторное пространство}%
   {Dstar vector space}%
\Index{texVectorSpace}%D%26
   {$D\star$\hyph произведение вектора на скаляр}%
   {Dstar product of vector over scalar, vector space}%
\Index{texCalculus}%D%96
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\SetIndexSpace%
\Index{texELie}%E%28
   {enhanced Lie group}%
   {enhanced Lie group}%
\Index{texDiffEq}%E%29
   {essential parameters}%
   {essential parameters}%
\SetIndexSpace%
\Index{texTypeBasis}%G%30
   {\Gbasis}%
   {G-basis}%
\Index{texTypeBasis}%G%31
   {\Gcoords ы}%
   {G-coordinates}%
\Index{texTypeBasis}%G%32
   {\Gspace о}%
   {GSpace}%
\Index{texBasis}%G%267
   {\Gbasis\ векторного пространства}%
   {G-basis}%
\Index{texBasis}%G%270
   {\Gcoords ы базиса}%
   {G-coordinates}%
\Index{texBasis}%G%271
   {\Gspace о}%
   {GSpace}%
\SetIndexSpace%
\Index{texPolymodule}%N%231
   {$(n)$\hyph векторное пространство}%
   {(n)-vector space}%
\Index{texBundleRelation}%N%218
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\SetIndexSpace%
\Index{texBiring}%R%35
   {\sups строка матрицы}%
   {r row}%
\Index{texVectorSpace}%R%36
   {\RC вырожденная матрица}%
   {RC singular matrix}%
\Index{texVectorSpace}%R%37
   {\RC главный минор}%
   {RC-major minor}%
\Index{texBiring}%R%38
   {\RC квазидетерминант}%
   {RC-quasideterminant}%
\Index{texVectorSpace}%R%39
   {\RC матричная группа}%
   {rc-matrix group}%
\Index{texVectorSpace}%R%40
   {\RC невырожденная матрица}%
   {RC nonsingular matrix}%
\Index{texBiring}%R%41
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index{texBiring}%R%42
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Index{texVectorSpace}%R%43
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Index{texBiring}%R%44
   {\RC степень}%
   {rc power}%
\Index{texVectorSpace}%R%45
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index{texVectorSpace}%R%213
   {$R\star$\Hyph модуль}%
   {Rstar-module}%
\Index{texBiring}%R%47
   {$r$\hyph строка матрицы}%
   {r-row}%
\SetIndexSpace%
\Index{texDrcMorphism}%S%314
   {$(S\RCstar,T\RCstar)$\Hyph линейное отображение векторных пространств}%
   {src trc linear map of vector spaces}%
\Index{texLinearMap}%S%48
   {$\star D$\Hyph произведением \drc линейного отображения $A$ на скаляр}%
   {starD product of drc linear map over scalar}%
\Index{texVectorSpace}%S%217
   {$\star D$\hyph векторное пространство}%
   {starD-vector space}%
\Index{texVectorSpace}%S%216
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index{texTstarRepresentation}%S%49
   {\sT сдвиг}%
   {starT shift}%
\Index{texFiberedGroup}%S%50
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\Index{texTstarMorphism}%S%160
   {\sT представление $\mathcal{F}$\Hyph алгебры $A$ в множестве $M$}%
   {starT representation of algebra}%
\Index{texFiberedAlgebra}%S%162
   {\sT представление расслоенной $\mathcal{F}$\Hyph алгебры}%
   {starT representation of fibered F-algebra}%
\Index{texFiberedGroup}%S%163
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index{texTstarMorphism}%S%308
   {\sT преобразование}%
   {starT transformation}%
\Index{texFiberedAlgebra}%S%167
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\SubIndex{}%71%
   {невырожденное}%
   {nonsingular transformation of bundle}%
\SetIndexSpace%
\Index{texVectorSpace}%T%51
   {\Ts векторное пространство матриц}%
   {matrices vector space}%
\Index{texVectorSpace}%T%52
   {\Ts линейная комбинация векторов}%
   {linear composition of  vectors}%
\Index{texFiberedGroup}%T%316
   {\Ts представление расслоенной группы}%
   {Tstar representation of fibered group}%
\Index{texTstarRepresentation}%T%53
   {\Ts сдвиг}%
   {Tstar shift}%
\Index{texTstarMorphism}%T%301
   {\Ts представление $\mathcal{F}$\Hyph алгебры $A$ в множестве $M$}%
   {Tstar representation of algebra}%
\Index{texFiberedAlgebra}%T%321
   {\Ts представление расслоенной $\mathcal{F}$\Hyph алгебры}%
   {Tstar representation of fibered F-algebra}%
\Index{texTstarMorphism}%T%309
   {\Ts преобразование}%
   {Tstar transformation}%
\Index{texFiberedAlgebra}%T%327
   {\Ts преобразование расслоения}%
   {Tstar transformation of bundle}%
\SetIndexSpace%
\Index{texNewton}%V%54
   {vector potential}%
   {vector potential}%
\SetIndexSpace%
\Index{texAffine}%А%56
   {автопараллельная кривая}%
   {auto parallel line}%
\Index{texDrcBasis}%А%57
   {активное \sT представление}%
   {active representation, vector space}%
\Index{texBasis}%А%262
   {активное представление}%
   {active representation}%
\Index{texBasis}%А%263
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index{texLie}%А%58
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\SubIndex{texLie}%9%
   {определённая слева}%
   {left defined algebra Lie}%
\SubIndex{texLie}%10%
   {определённая справа}%
   {right defined algebra Lie}%
\Index{texBiring}%А%59
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index{texFiberedGroup}%А%60
   {антигомоморфизм расслоенных групп}%
   {antihomomorphism of fibered groups}%
\Index{texBundleRelation}%А%156
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index{texFiberedAlgebra}%А%61
   {арность операции}%
   {arity of operation}%
\Index{texBasis}%А%277
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index{texBasis}%А%275
   {аффинный базис}%
   {Affine Basis}%
\SetIndexSpace%
\Index{texCartesian}%Б%172
   {база отображения}%
   {base of map}%
\Index{texBundleRelation}%Б%233
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index{texTypeBasis}%Б%16
   {базис}%
   {}%
\SubIndex{texTypeBasis}%1%
   {аффинный}%
   {Affine Basis}%
\SubIndex{texTypeBasis}%2%
   {ортонормальный}%
   {Orthonornal Basis}%
\SubIndex{texTypeBasis}%3%
   {центро-аффинный}%
   {Central Affine Basis}%
\Index{texBasis}%Б%266
   {базис векторного пространства}%
   {Basis}%
\Index{texLieRepresentation}%Б%62
   {базовый вектор}%
   {}%
\SubIndex{texLieRepresentation}%11%
   {\sT представления}%
   {basis vector of starT representation}%
\SubIndex{texLieRepresentation}%12%
   {\Ts представления}%
   {basis vector of Tstar representation}%
\Index{texLie}%Б%63
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index{texLieRepresentation}%Б%64
   {бесконечно малый генератор}%
   {infinitesimal generator}%
\Index{texBiring}%Б%65
   {бикольцо}%
   {biring}%
\SetIndexSpace%
\Index{texPolymodule}%В%230
   {($D_1\RCstar$, ..., $D_n\RCstar$)\hyph векторное пространство}%
   {(d1rc,dnrc)-vector space}%
\Index{texPolymodule}%В%229
   {($S\star$, $\star T$)\hyph векторное пространство}%
   {(Sstar,starT)-vector space}%
\Index{texDiffProperty}%В%69
   {вектор Килинга второго рода}%
   {Killing vector second type}%
\Index{texRepresentation}%В%261
   {вектор\hyph столбец}%
   {column vector}%
\Index{texFiberedAlgebra}%В%70
   {векторное расслоение}%
   {vector bundle}%
\Index{texRepresentation}%В%260
   {вектор\hyph строка}%
   {row vector}%
\Index{texDiffEq}%В%71
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index{texNewton}%В%72
   {второй закон Ньютона}%
   {Second Newton law}%
\SetIndexSpace%
\Index{texDrcBasis}%Г%73
   {геометрический объект}%
   {}%
\SubIndex{texDrcBasis}%13%
   {в координатном представлении,	определённом в векторном пространстве}%
   {geometrical object, coordinate vector space}%
\SubIndex{texDrcBasis}%14%
   {определённый в векторном пространстве}%
   {geometrical object, vector space}%
\SubIndex{texDrcBasis}%15%
   {типа $A$}%
   {geometrical object of type A, vector space}%
\Index{texBasis}%Г%290
   {геометрический объект в векторном пространстве}%
   {geometrical object, vector space}%
\Index{texBasis}%Г%288
   {геометрический объект в координатном представлении}%
   {geometrical object, coordinate vector space}%
\Index{texBasis}%Г%293
   {геометрический объект типа $A$ в векторном пространстве}%
   {geometrical object of type A, vector space}%
\Index{texReferenceFrame}%Г%74
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index{texFiberedAlgebra}%Г%75
   {гомоморфизм расслоенных $\mathcal{F}$\Hyph алгебр}%
   {homomorphism of fibered F-algebras}%
\Index{texFiberedGroup}%Г%76
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index{texTypeBasis}%Г%77
   {группа аффинных преобразований}%
   {AffineTransformationGroup}%
\Index{texBasis}%Г%274
   {группа аффинных преобразований}%
   {AffineTransformationGroup}%
\Index{texBasis}%Г%264
   {группа симметрии}%
   {symmetry group}%
\Index{texDrcBasis}%Г%78
   {группа симметрии}%
   {SymmetryGroup}%
\Index{texGroupRing}%Г%79
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index{}%Д%283
   {движение на многообразии базисов}%
   {movement transformation}%
\Index{texCartesian}%Д%331
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index{texCartesian}%Д%176
   {декартова степень расслоения}%
   {Cartesian power of bundle}%
\Index{texCartesian}%Д%180
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index{texCartesian}%Д%181
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index{texBundleRelation}%Д%113
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index{texBundleRelation}%Д%227
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index{texCalculus}%Д%105
   {дифференциал отображения нормированного \drc векторного пространства в нормированное тело}%
   {differential, drc vector space to skew field}%
\Index{texCalculus}%Д%99
   {дифференцируемая функция \drc векторного пространства в тело $D$ }%
   {differentiable functions, drc vector space to skew field}%
\SetIndexSpace%
\Index{texDrcMorphism}%З%312
   {закон ассоциативности для \drc линейных отображений векторных пространств}%
   {associative law for drc linear maps of vector spaces}%
\Index{texVectorSpace}%З%310
   {закон ассоциативности для \Ts векторного пространства}%
   {associative law, Tstar vector space}%
\Index{texTstarRepresentation}%З%80
   {закон ассоциативности для ковариантного \Ts представления}%
   {associative law for Tstar covariant representation}%
\Index{texLinearMap}%З%311
   {закон ассоциативности для парных представлений}%
   {associative law for twin representations}%
\Index{texBundleRelation}%З%155
   {закон ассоциативности произведения расслоенных соответствий}%
   {associative law, composition of fibered correspondences}%
\Index{texVectorSpace}%З%81
   {закон дистрибутивности}%
   {}%
\SubIndex{texVectorSpace}%20%
   {\Ts векторное пространство}%
   {distributive law, Tstar vector space}%
\Index{texVectorSpace}%З%82
   {закон унитарности}%
   {}%
\SubIndex{texVectorSpace}%21%
   {для \Ts векторного пространства}%
   {unitarity law, Tstar vector space}%
\SetIndexSpace%
\Index{texFiberedAlgebra}%И%84
   {изоморфизм расслоенных алгебр}%
   {isomorphism of fibered F-algebras}%
\Index{texLinearLie}%И%85
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index{texHomotopy}%К%4
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index{texBundleRelation}%К%111
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index{texBundleRelation}%К%112
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index{texBasis}%К%278
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index{texBasis}%К%284
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index{texFiberedGroup}%К%318
   {ковариантное \Ts представление расслоенной группы}%
   {Tstar covariant representation of fibered group}%
\Index{texBundleRelation}%К%228
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index{texCartesian}%К%332
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index{texFiberedGroup}%К%317
   {контравариантное \Ts представление расслоенной группы}%
   {Tstar contravariant representation of fibered group}%
\Index{texVectorSpace}%К%21
   {координатная матрица}%
   {}%
\SubIndex{texVectorSpace}%6%
   {вектора в \drc базисе}%
   {coordinate matrix of vector in drc basis}%
\SubIndex{texVectorSpace}%7%
   {множества векторов в векторном пространстве \dcr строк}%
   {coordinate matrix of set of vectors, dcr vector space}%
\SubIndex{texVectorSpace}%8%
   {множества векторов в векторном пространстве \drc строк}%
   {coordinate matrix of set of vectors, drc vector space}%
\Index{texReferenceFrame}%К%86
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index{texGenRelativity}%К%239
   {координатная система отсчёта в пространстве событий}%
   {coordinate reference frame in event space}%
\Index{texBasis}%К%285
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index{texDrcBasis}%К%88
   {координатное представление в \drc векторном пространстве}%
   {coordinate representation, vector space}%
\Index{texBasis}%К%287
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index{texBasis}%К%286
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index{texVectorSpace}%К%89
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index{texVectorSpace}%К%22
   {координаты вектора в \drc базисе}%
   {coordinates of vector in drc basis}%
\Index{texDrcBasis}%К%90
   {координаты геометрического объекта}%
   {}%
\SubIndex{texDrcBasis}%22%
   {в векторном пространстве}%
   {coordinates of geometrical object, vector space}%
\SubIndex{texDrcBasis}%23%
   {в координатном векторном пространстве}%
   {coordinates of geometrical object, coordinate vector space}%
\Index{texBasis}%К%291
   {координаты геометрического объекта}%
   {coordinates of geometrical object, vector space}%
\Index{texBasis}%К%289
   {координаты геометрического объекта в координатном представлении}%
   {coordinates of geometrical object, coordinate vector space}%
\Index{texVectorSpace}%К%91
   {координаты множества векторов в \dcr векторном пространстве}%
   {coordinates of set of vectors, dcr vector space}%
\Index{texVectorSpace}%К%92
   {координаты множества векторов в \drc векторном пространстве}%
   {coordinates of set of vectors, drc vector space}%
\Index{texDrcBasis}%К%93
   {координаты представления}%
   {coordinates of representation}%
\Index{texBasis}%К%265
   {координаты представления}%
   {coordinates of representation}%
\Index{texAffine}%К%94
   {кривизна Картана}%
   {Cartan curvature}%
\Index{texAffine}%К%95
   {кручение}%
   {torsion}%
\SetIndexSpace%
\Index{texVectorSpace}%Л%98
   {левое векторное пространство}%
   {left vector space}%
\Index{texLie}%Л%101
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index{texRepresentation}%Л%247
   {левостороннее ковариантное представление группы}%
   {left-side covariant representation}%
\Index{texRepresentation}%Л%249
   {левостороннее контравариантное представление группы}%
   {left-side contravariant representation}%
\Index{texTstarMorphism}%Л%302
   {левостороннее представление $\mathcal{F}$\Hyph алгебры $A$ в множестве $M$}%
   {left-side representation of algebra}%
\Index{texRepresentation}%Л%244
   {левостороннее представление группы}%
   {left-side representation of group}%
\Index{texFiberedAlgebra}%Л%322
   {левостороннее представление расслоенной $\mathcal{F}$\Hyph алгебры}%
   {left-side representation of fibered F-algebra}%
\Index{texTstarMorphism}%Л%164
   {левостороннее преобразование}%
   {left-side transformation}%
\Index{texFiberedAlgebra}%Л%328
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index{texLie}%Л%103
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index{texVectorSpace}%Л%214
   {левый модуль}%
   {left module}%
\Index{texTstarRepresentation}%Л%108
   {левый сдвиг}%
   {left shift}%
\Index{texRepresentation}%Л%251
   {левый сдвиг на группе}%
   {left shift, group}%
\Index{texFiberedGroup}%Л%109
   {левый сдвиг на расслоении групп}%
   {Tstar shift, fibered group}%
\Index{texReferenceFrame}%Л%110
   {линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index{texRepresentation}%Л%240
   {линейное представление группы}%
   {linear representation of group}%
\Index{texCartesian}%Л%116
   {лифт отображения}%
   {lift of map}%
\Index{texBundleRelation}%Л%232
   {лифт соответствия}%
   {lift of correspondence}%
\Index{texReferenceFrame}%Л%117
   {локальная система отсчёта}%
   {local reference frame}%
\SetIndexSpace%
\Index{texDrcMorphism}%М%118
   {матрица \drc линейного отображения}%
   {matrix of drc linear map}%
\Index{texAffine}%М%119
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index{texDrcBasis}%М%120
   {многообразие базисов}%
   {}%
\SubIndex{texDrcBasis}%24%
   {\drc векторного пространства}%
   {basis manifold of vector space}%
\SubIndex{texTypeBasis}%25%
   {аффинного пространства}%
   {Basis Manifold, Affine Space}%
\SubIndex{texTypeBasis}%26%
   {евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\SubIndex{texTypeBasis}%27%
   {центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index{texBasis}%М%276
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index{texBasis}%М%268
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Index{texBasis}%М%282
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index{texBasis}%М%280
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index{texReferenceFrame}%М%123
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index{texTstarMorphism}%М%298
   {морфизм \Ts представлений $\mathcal{F}$\Hyph алгебры}%
   {morphism of representations of F algebra}%
\Index{texTstarMorphism}%М%300
   {морфизм \Ts представлений $\mathcal{F}$\Hyph алгебры в $\mathcal{H}$\Hyph алгебре}%
   {morphism of representations of F algebra in H algebra}%
\Index{texTstarMorphism}%М%307
   {морфизм \Ts представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\SetIndexSpace%
\Index{texVectorSpace}%Н%124
   {невырожденная система \drc линейных уравнений}%
   {nonsingular system of linear equations}%
\Index{texRepresentation}%Н%241
   {невырожденное \Ts преобразование}%
   {nonsingular transformation}%
\Index{texReferenceFrame}%Н%125
   {неголономная координата}%
   {anholonomic coordinate}%
\Index{texReferenceFrame}%Н%126
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index{texReferenceFrame}%Н%127
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index{texAffine}%Н%128
   {неметричность}%
   {nonmetricity}%
\Index{texCalculus}%Н%97
   {норма на \drc векторном пространстве}%
   {norm on drc vector space}%
\Index{texCalculus}%Н%100
   {норма на теле}%
   {absolute value on skew field}%
\Index{texCalculus}%Н%102
   {нормированное тело}%
   {valued skew field}%
\Index{texCalculus}%Н%104
   {нормированным \drc векторное пространство}%
   {normed drc vector space}%
\SetIndexSpace%
\Index{texBundleRelation}%О%121
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index{texBundleRelation}%О%115
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index{texBiring}%О%129
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index{texReferenceFrame}%О%130
   {объект неголономности}%
   {anholonomity object}%
\Index{texTstarRepresentation}%О%131
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index{texRepresentation}%О%259
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index{texFiberedGroup}%О%132
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index{texTstarMorphism}%О%303
   {однотранзитивное представление алгебры $A$}%
   {single transitive representation of algebra}%
\Index{texRepresentation}%О%258
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index{texFiberedAlgebra}%О%323
   {однотранзитивное представление расслоенной $\mathcal{F}$\Hyph алгебры}%
   {single transitive representation of fibered F-algebra}%
\Index{texFiberedAlgebra}%О%133
   {операция на расслоении}%
   {operation on bundle}%
\Index{texBiring}%О%134
   {определитель матрицы}%
   {determinant}%
\Index{texTstarRepresentation}%О%135
   {орбита \Ts представления группы}%
   {orbit of representation of group}%
\Index{texRepresentation}%О%253
   {орбита представления группы}%
   {orbit of representation of group}%
\Index{texFiberedGroup}%О%136
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index{texBasis}%О%281
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Index{texTidal}%О%137
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index{texReferenceFrame}%О%138
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\SetIndexSpace%
\Index{texReferenceFrame}%П%139
   {параллелограм}%
   {parallelogram}%
\Index{texTstarRepresentation}%П%140
   {парные представления группы}%
   {twin representations of group}%
\Index{texFiberedGroup}%П%319
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index{texLinearMap}%П%320
   {парные представления тела}%
   {twin representations of skew field}%
\Index{texDrcBasis}%П%141
   {пассивное \Ts представление}%
   {passive representation}%
\Index{texBasis}%П%273
   {пассивное представление}%
   {passive representation}%
\Index{texBasis}%П%272
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index{texNewton}%П%142
   {первый закон Ньютона}%
   {First Newton law}%
\Index{texAffine}%П%143
   {перенос Картана}%
   {Cartan transport}%
\Index{texAffine}%П%144
   {перенос Френе}%
   {Frenet transport}%
\Index{texBundleRelation}%П%220
   {подрасслоение}%
   {subbundle}%
\Index{texNewton}%П%146
   {потенциальная энергия}%
   {potential energy}%
\Index{texVectorSpace}%П%149
   {правое векторное пространство}%
   {right vector space}%
\Index{texLie}%П%151
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index{texRepresentation}%П%248
   {правостороннее ковариантное представление группы}%
   {right-side covariant representation}%
\Index{texRepresentation}%П%250
   {правостороннее контравариантное представление группы}%
   {right-side contravariant representation}%
\Index{texTstarMorphism}%П%304
   {правостороннее представление $\mathcal{F}$\Hyph алгебры $A$ в множестве $M$}%
   {right-side representation of algebra}%
\Index{texRepresentation}%П%245
   {правостороннее представление группы}%
   {right-side representation of group}%
\Index{texFiberedAlgebra}%П%324
   {правостороннее представление расслоенной $\mathcal{F}$\Hyph алгебры}%
   {right-side representation of fibered F-algebra}%
\Index{texTstarMorphism}%П%242
   {правостороннее преобразование}%
   {right-side transformation}%
\Index{texRepresentation}%П%243
   {правостороннее преобразование}%
   {right-side transformation}%
\Index{texLie}%П%153
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index{texVectorSpace}%П%215
   {правый модуль}%
   {right module}%
\Index{texTstarRepresentation}%П%158
   {правый сдвиг}%
   {right shift}%
\Index{texRepresentation}%П%252
   {правый сдвиг на группе}%
   {right shift, group}%
\Index{texBasis}%П%292
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometrical object, vector space}%
\Index{texDrcBasis}%П%159
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometrical object, vector space}%
\Index{texTstarRepresentation}%П%161
   {представление группы}%
   {}%
\SubIndex{texDrcBasis}%38%
   {\drc линейное \sT}%
   {linear representation of group}%
\SubIndex{texDrcBasis}%39%
   {\rcd}%
   {rcd linear representation of group}%
\SubIndex{texTstarRepresentation}%40%
   {\sT}%
   {starT representation of group}%
\SubIndex{texTstarRepresentation}%41%
   {\Ts}%
   {Tstar representation of group}%
\SubIndex{texTstarRepresentation}%42%
   {ковариантное \Ts}%
   {Tstar covariant representation of group}%
\SubIndex{texTstarRepresentation}%43%
   {контравариантное \Ts}%
   {Tstar contravariant representation of group}%
\SubIndex{texTstarRepresentation}%44%
   {эффективное}%
   {effective representation of group}%
\Index{texRepresentation}%П%246
   {представление группы}%
   {representation of group}%
\Index{texGenRelativity}%П%165
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index{texTstarMorphism}%П%313
   {преобразование множества}%
   {transformation of set}%
\Index{texDrcBasis}%П%166
   {преобразование на многообразии базисов}%
   {}%
\SubIndex{texDrcBasis}%62%
   {активное}%
   {active transformation, vector space}%
\SubIndex{texTypeBasis}%63%
   {аффинное}%
   {affine transformation}%
\SubIndex{texTypeBasis}%64%
   {движение}%
   {movement transformation}%
\SubIndex{texTypeBasis}%65%
   {квазиаффинное}%
   {quasi affine transformation}%
\SubIndex{texTypeBasis}%66%
   {квазидвижение}%
   {quasi movement}%
\SubIndex{texDrcBasis}%67%
   {пассивное}%
   {passive transformation, vector space}%
\Index{texFiberedAlgebra}%П%329
   {преобразование расслоения}%
   {transformation of bundle}%
\Index{texCartesian}%П%221
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index{texCartesian}%П%222
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index{texBundleRelation,texBundleRelation}%П%225
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\mathcal{B}$}%
   {reduced fibered correspondence from A to B}%
\Index{texBundleRelation}%П%226
   {приведенное расслоенное соответствие в $\mathcal{A}$}%
   {reduced fibered correspondence in A}%
\Index{texBiring}%П%168
   {приводимое бикольцо}%
   {reducible biring}%
\Index{texBiring}%П%169
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index{texBiring}%П%170
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index{texDrcBasis}%П%171
   {принцип инвариантности}%
   {invariance principle}%
\Index{texBasis}%П%296
   {принцип инвариантности в векторном пространстве}%
   {invariance principle, vector space}%
\Index{texBundleRelation}%П%235
   {продолжение соответствия}%
   {extension of correspondence}%
\Index{texDrcBasis}%П%173
   {произведение геометрического объекта и константы}%
   {product of geometrical object and constant}%
\Index{texBasis}%П%295
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometrical object and constant, vector space}%
\Index{texTstarMorphism}%П%299
   {произведение морфизмов \Ts представлений $\mathcal{F}$\Hyph алгебры}%
   {product of morphisms of representations of F algebra}%
\Index{texBundleRelation}%П%154
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index{texBundleRelation}%П%188
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\SubIndex{texVectorSpace}%74%
   {\drc линейных уравнений}%
   {extended matrix, system of drc linear equations}%
\SubIndex{texVectorSpace}%75%
   {\rcd линейных уравнений}%
   {extended matrix, system of rcd linear equations}%
\Index{texAffine}%П%174
   {производная Картана}%
   {Cartan derivative}%
\Index{texDiffProperty}%П%175
   {производная Ли}%
   {Lie derivative}%
\SubIndex{texDiffProperty}%72%
   {метрики}%
   {Lie derivative of metric}%
\SubIndex{texDiffProperty}%73%
   {связности}%
   {Lie derivative of connection}%
\Index{texCartesian}%П%333
   {пространство отображений}%
   {mapping space}%
\Index{texBundleRelation}%П%236
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index{texLieRepresentation}%П%177
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index{texTstarRepresentation}%П%178
   {прямое произведение \Ts представлений группы}%
   {direct product of representations of group}%
\Index{texRepresentation}%П%254
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index{texFiberedGroup}%П%179
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index{texReferenceFrame}%П%182
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index{texVectorSpace}%Р%183
   {размерность \drc векторного пространства}%
   {dimension of vector space}%
\Index{texFiberedAlgebra}%Р%184
   {расслоенная $\mathcal{F}$\Hyph алгебра}%
   {fibered F-algebra}%
\Index{texFiberedAlgebra}%Р%186
   {расслоенная $\mathcal{F}$\Hyph подалгебра}%
   {fibered F-subalgebra}%
\Index{texFiberedAlgebra}%Р%185
   {расслоенная группа}%
   {fibered group}%
\Index{texBundleRelation}%Р%145
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index{texBundleRelation}%Р%237
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index{texBundleRelation}%Р%238
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index{texFiberedAlgebra}%Р%187
   {расслоенное кольцо}%
   {fibered ring}%
\Index{texBundleRelation}%Р%219
   {расслоенное подмножество}%
   {fibered subset}%
\Index{texBundleRelation}%Р%224
   {расслоенное соответствие в $\mathcal{A}$}%
   {fibered correspondence in A}%
\Index{texBundleRelation}%Р%330
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index{texBundleRelation}%Р%223
   {расслоенное соответствие из $\mathcal{A}$ в $\mathcal{B}$}%
   {fibered correspondence from A to B}%
\Index{texBundleRelation}%Р%157
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\SetIndexSpace%
\Index{texAffine}%С%189
   {связность Картана}%
   {Cartan connection}%
\Index{texAffine}%С%190
   {символ Картана}%
   {Cartan symbol}%
\Index{texBiring}%С%191
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index{texBundleRelation}%С%148
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index{texGenRelativity}%С%192
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index{texVectorSpace}%С%193
   {система \drc линейных уравнений}%
   {system of linear equations}%
\Index{texGenRelativity}%С%194
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index{texReferenceFrame}%С%195
   {система отсчёта на многообразии}%
   {reference frame}%
\Index{texNewton}%С%196
   {скалярный потенциал}%
   {scalar potential}%
\Index{texTidal}%С%197
   {скорость отклонения}%
   {speed of deviation}%
\Index{texBundleRelation}%С%297
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index{texBiring}%С%198
   {стандартное представление матрицы}%
   {Standard representation}%
\Index{texDrcBasis}%С%199
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index{texBasis}%С%269
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index{texBundleRelation}%С%234
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index{texLinearMap}%С%200
   {сумма \drc линейных отображений}%
   {sum of drc linear maps, drc vector spaces}%
\Index{texDrcBasis}%С%201
   {сумма геометрических объектов}%
   {sum of geometrical objects}%
\Index{texBasis}%С%294
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometrical objects, vector space}%
\SetIndexSpace%
\Index{texNewton}%Т%202
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index{texLie}%Т%203
   {тензорное произведение представлений}%
   {tensor product of representations}%
\Index{texVectorSpace}%Т%204
   {тип векторного пространства}%
   {vector space type}%
\Index{texReferenceFrame}%Т%205
   {типа $G$ система отсчёта}%
   {type G reference frame}%
\Index{texCalculus}%Т%152
   {топологическое \drc векторное пространство}%
   {topological drc vector space}%
\Index{texCalculus}%Т%33
   {топологическое тело}%
   {topological skew field}%
\Index{texBundleRelation}%Т%147
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index{texTstarMorphism}%Т%305
   {транзитивное представление алгебры $A$}%
   {transitive representation of algebra}%
\Index{texRepresentation}%Т%257
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index{texFiberedAlgebra}%Т%325
   {транзитивное представление расслоенной $\mathcal{F}$\Hyph алгебры}%
   {transitive representation of fibered F-algebra}%
\SetIndexSpace%
\Index{texDiffProperty}%У%206
   {уравнение Килинга}%
   {Killing equation}%
\Index{texDiffProperty}%У%207
   {уравнение Килинга второго рода}%
   {Killing equation second type}%
\Index{texBiring}%У%208
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index{texCalculus}%Ф%150
   {функция $\gi n$ $D$\Hyph значных переменных}%
   {function of n D valued variables}%
\Index{texCalculus}%Ф%68
   {функция, непрерывная по совокупности аргументов}%
   {function continuous with respect to set of arguments}%
\SetIndexSpace%
\Index{texBasis}%Ц%279
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index{texCalculus}%Ч%106
   {частная производная отображения $f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping with respect to variable, skew field}%
\Index{texCalculus}%Ч%107
   {частная производная отображения $\Vector f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping with respect to variable, drc vector space}%
\SetIndexSpace%
\Index{texAffine}%Э%209
   {экстремальная кривая}%
   {extreme line}%
\Index{texTstarMorphism}%Э%306
   {эффективное представление алгебры $A$}%
   {effective representation of algebra}%
\Index{texRepresentation}%Э%256
   {эффективное представление группы}%
   {effective representation of group}%
\Index{texFiberedAlgebra}%Э%326
   {эффективное представление расслоенной $\mathcal{F}$\Hyph алгебры}%
   {effective representation of fibered F-algebra}%
\Index{texFiberedGroup}%Э%315
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index{texVectorSpace}%Э%210
   {эффективное представление тела}%
   {effective representation of skew field}%
\SetIndexSpace%
\Index{texTstarRepresentation}%Я%211
   {ядро неэффективности \Ts представления группы $G$}%
   {kernel of inefficiency of representation of group}%
\Index{texRepresentation}%Я%255
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index{texFiberedGroup}%Я%212
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%

\CloseIndex


==> Preface.Algebra.Russian.tex <==
%auto-ignore
\def\texPreface_Algebra{}
\ifx\texPrefaceRelation\Defined
\ifx\PrintBook\Defined
				\chapter{Предисловие}
%\else
%			\section{Предисловие}
\fi
\epigraph{Кто-то из посетителей Ясной Поляны обвинил Толстого в том,
что он жестоко поступил с Анной Карениной
заставив ее броситься под поезд.
//
Толстой улыбнулся и ответил:
//
- Это мнение
напоминает мне случай с Пушкиным. Однажды он сказал
кому-то из своих приятелей: «Представь, какую штуку удрала со мной Татьяна.
Она замуж вышла. Этого я никак не ожидал от нее». То же самое и я могу сказать
про Анну Каренину. Вообще герои и героини мои делают иногда такие штуки, каких я
не желал бы! Они делают то, что должны делать в действительной жизни и
как бывает в действительной жизни, а не то, что мне хочется.}
{\citeBib{Tolstoi about Anna Karenina}, с. 517}
\fi

\ifx\texPrefaceAlgebra\Defined
Теория представления алгебры имеет длинную и богатую историю.
На протяжении XX столетия теория представления стала неотъемлемой частью многих
приложений. Переход от алгебры к расслоенной алгебре открывает новые возможности.
Я предпринял попытку написать эту
\ifx\PrintBook\Defined
книгу
\else
статью
\fi
с целью увидеть новые свойства
расслоенной алгебры.
\fi

\ifx\texPrefaceRelation\Defined
Эта история началась много лет назад. В 15 лет у меня появились карманные деньги на
расход.
Я стал покупать книги по математике и физике. К тому моменту,
когда я поступил в университет, я собрал библиотеку любимых книг.
Среди этих книг была книга "Универсальная алгебра" Кона
(\citeBib{Cohn: Universal Algebra}),
которая чудом задержалась в магазине. Я не очень задумывался, что мне
ещё рано читать об этом. Читая эту книгу я полюбил алгебру.
Однако свою жизнь и исследование я посвятил геометрии, работая
на стыке геометрии и физики.

Спустя более чем 30 лет, я вдруг вернулся к этой книге. Мне стало любопытно,
что будет, если универсальная алгебра определена в слое расслоения.
Когда я начал писать статью \citeBib{0702.561} меня не покидало
ощущение, что нечто подобное я читал в молодости. Я разыскал книгу,
которая, как я полагал, была первоисточником. Но в этой книге были только
векторные расслоения. Но лишь, когда я начал писать эту статью, я окончательно
понял, что ничего подобного я не читал. Я не смог бы пройти мимо подобных фактов.

Выходит, что в молодости я об этом думал. Но почему я ждал столько лет?
И почему именно сейчас я начал это исследование? На первый вопрос я никогда
не найду ответа. А ответ на второй вопрос очень прост.
На протяжении многих лет я изучал систему отсчёта в общей теории относительности.
При этом меня интересовал не только классический случай, но и возможные отклонения
геометрии. Результаты, полученные в \citeBib{0702.561}, показали,
что в области моего исследования есть ещё много оставшихся без ответа вопросов.

Я планировал посвятить эту статью изучению
расслоенного отношения эквивалентности, так как оно представляет для меня
определённый интерес в будущем.
Однако необходимость дать чёткие формулировки вовлекла новые определения.
Дальше события приняли совершено не предсказуемый оборот.
Статья, которая планировалась быть предельно короткой
и занять месяц работы, безжалостно отнимает у меня время, меняет название
и направление исследования.\footnote{Азарт
охоты - одна из самых сильных страстей человечества.
Я ловлю себя на том, что я постоянно решаю новые для меня задачи.}
Статья, посвящённая расслоенному отношению эквивалентности, превращается в статью,
посвящённую расслоенным бинарным отношениям.

Расслоенное отношение - пожалуй одна из самых тонких тем в теории расслоенной
алгебры. Определение операции практически однозначно переносится на расслоения, так как
операция является отображением, и относительно нетрудно распространить операцию на сечения
и, если надо, потребовать непрерывность. Отношение - это подмножество
декартового произведения.
Если мы просто определим его послойно, то скорее всего мы потеряем связь между слоями.

Я решил полностью повторить путь, который необходим для определения отношения в
универсальной алгебре.
Когда я начал изучать расслоенные соответствия, я понял, что многие
формулировки в \citeBib{0702.561} должны быть изменены.
Определение
\xRef{0702.561}{definition: reduced Cartesian product of bundle}
порождает слишком тесные рамки
для определения расслоенных соответствий.
Определение, задающее соответствие только в слое, может и хорошо в некоторых
случаях\footnote{В частности, мы определяем расслоенное отношение,
определяя отношение в слое}, но за бортом остаются
расслоенные морфизмы. Анализ сложившейся ситуации разоблачает миф, с которым
я спокойно жил все годы. Точнее, я всегда пытался понять,
что из себя представляет база послойного отображения.
Является ли это отображение инъекцией, или оно
может быть произвольным. Ни одно определение
не даёт ясного ответа на этот вопрос. Для простоты восприятия я полагал, что
база послойного отображения
является инъекцией. На самом деле, раз характер отображения базы не оговорен,
это отображение может быть произвольным. Это приводит к более широкому
определению (определение
\xRef{0702.561}{definition: Cartesian product of bundle}) декартова произведения расслоений.
С другой стороны, определение
\xRef{0702.561}{definition: Cartesian product of bundle} приводит к
трудностям в определении расслоенных алгебр. Это приводит к необходимости
пользоваться двумя определениями декартова произведения расслоения.
Аналогичные соображения приводят к двум определениям расслоенного соответствия.

В конце концов я вернулся к отношению эквивалентности. Но мой труд
не пропал даром. Мой взгляд на проблему изменился.

Из определения \ref{definition: Fibered Correspondence}
следует, что понятие непрерывности является существенной компонентой
определения расслоенного соответствия. Вслед за этим определением
я разъясняю, что означает непрерывность соответствия.
\fi

%В отличие от операций, отношения в расслоенной алгебре имеет меньше свойств.
%Тем не менее некоторые важные свойства сохраняются.
%Отношение эквивалентности играет большую роль в различных разделах математики.

\ifx\texPrefaceAlgebra\Defined
Так как сечения расслоения
может быть не определено на всём расслоении, все утверждения предполагают
некоторую область определения.
Подобные утверждения строятся по образцу утверждения
о существовании тривиального касательного расслоения на многообразии.

Однако существует другая группа утверждений, ограничивающих область
определения расслоенной
$\mathcal{F}$\Hyph алгебры. В тексте приведены соответствующие примеры.
Данная ситуация сводится к следующему.

Преобразование слоя при параллельном переносе предполагается
взаимно однозначным отображением.
Непрерывно перемещаясь вдоль базы,
мы непрерывно переходим от слоя к другому.
Предположение, что отображение между слоями является гомеоморфизмом,
гарантирует непрерывную деформацию слоя.

Если мы выберем точку в слое, то её траектория при движении проекции вдоль
базы будет паралельна базе. В дифференциальной
геометрии подобные кривые называются горизонтальными.
Мы так же будем придерживаться этого термина.

Если мы предполагаем на слое структуру
$\mathcal{F}$\Hyph алгебры, то соответствующее отображение
должно быть изоморфизмом $\mathcal{F}$\Hyph алгебры.
Непрерывность позволяет сохранить при параллельном переносе
изучаемые конструкции, сделать переход от слоя к слою
практически незаментным.

Эта картина хорошо работает в малом. Когда мы переходим к
конечным отрезкам на базе,
непрерывность становится ответственной за то,
что мы не можем продлить структуру $\mathcal{F}$\Hyph алгебры
сколь угодно далеко.
Например,  могут появиться точки, где гомеоморфизм может
быть нарушен. Это происходит, когда пересекаются горизонтальные кривые или
изменяются топологические свойства слоя. Соответствующий слой мы
называем вырожденным, а его проекцию - точкой вырождения.

Вопрос о том, как много точек вырождения, вообще говоря, непростой.
Интуитивно ясно, что это множество невелико по сравнению с базой.
Тем не менее, это множество может оказаться существенным
для изучения геометрии расслоения или физических процессов,
связанных с этим расслоением.

К подобным явлениям в теории дифференциальных уравнений
относится задача продления решения дифференциального уравнения.
В тоже время, дифференциальное уравнение может иметь два типа решения.
Регулярное рещение принадлежит некоторому семейству
функций, зависящих от произвольных постоянных.
Особое решение является огибающей семейства регулярных решений.

Задача описания слоёв расслоения, независимо от того вырождены
они или нет, имеет интересное решение. Любой путь на базе расслоения
является отображением отрезка $I=[0,1]$ в базу расслоения.
Мы можем предположить, что слои расслоения не гомеоморфны,
но гомотопны.

Группа голономий расслоения также накладывает ограничение
на структуру расслоенной $\mathcal F$\Hyph алгебры
$\mathcal A=\bundle{}pA{}$. Естественно предположить, что при
параллельном переносе мы гомоморфно отображаем
$\mathcal F$\Hyph алгебру из одного слоя в другой.
Следовательно, предполагается, что преобразование, порождённое
параллельным переносом вдоль замкнутого контура
является гомоморфизмом $\mathcal F$\Hyph алгебры. Таким образом, всё хорошо,
если группа голономий расслоения $\mathcal A$ является
подгруппой группы гомоморфизмов $\mathcal F$\Hyph алгебры
$A$. В этом случае мы будем называть
расслоенную $\mathcal F$\Hyph алгебру $\mathcal A$
голономной.
В противном случае мы будем называть
расслоенную $\mathcal F$\Hyph алгебру $\mathcal A$
неголономной.

Из теории векторных расслоений известно, что не
не всякая расслоенная $\mathcal F$\Hyph алгебра
является голономной. В тоже время, теория векторных расслоений
предлагает рецепт каким образом мы можем работать с
неголономной расслоенной $\mathcal F$\Hyph алгеброй.

Это замечание относится также к теории представления
расслоенной $\mathcal F$\Hyph алгебры.

Чтобы сделать новые конструкции более наглядными,
я строю соответствующие диаграммы.
\fi

%Я следую соглашениям.
Обозначения операций и отношений по возможности
сохраняются как они введены в теории множеств. Это не приводит к
недоразумениям, так как обозначения расслоений отличны от обозначений
множеств. Для обозначения расслоения и слоя я буду пользоваться одной
и той же буквой в разных алфавитах.

Проекция расслоения, сечение, морфизм расслоений предполагаются непрерывными отображениями.


==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%
\Symb{texBiring}%
   {$(^{\gi a}_{\gi b})$\hyph\CR квазидетерминант}%
   {a b CR quasideterminant definition}%
\Symb{texBiring}%
   {$(^{\gi a}_{\gi b})$\hyph \RC квазидетерминант}%
   {a b RC-quasideterminant definition}%
\Symb{texBiring}%
   {минор}%
   {A from b a}%
\Symb{texBiring}%
   {минор}%
   {A from columns T}%
\Symb{texBiring}%
   {минор}%
   {A from rows S}%
\Symb{texBiring}%
   {минор}%
   {A without column a}%
\Symb{texBiring}%
   {минор}%
   {A without columns T}%
\Symb{texBiring}%
   {минор}%
   {A without row b}%
\Symb{texBiring}%
   {минор}%
   {A without rows S}%
\Symb{texPolymodule}%
   {активное преобразование}%
   {active transformation}%
\Symb{texTypeBasis}%
   {аффинное пространство}%
   {affine space}%
\Symb{texBasis}%
   {аффинное пространство}%
   {An}%
\Symb{texBiring}%
   {\subs строка ($c$\hyph строка) матрицы}%
   {c row}%
\Symb{texBiring}%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
\Symb{texBiring}%
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Symb{texBiring}%
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Symb{texVectorSpace}%
   {\dcr вектор}%
   {dcr vector}%
\Symb{texLie}%
   {производная левого сдвига}%
   {derivative of left shift}%
\Symb{texLie}%
   {производная левого сдвига}%
   {derivative of left shift, 1-Parameter Group}%
\Symb{texLie}%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb{texLie}%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb{texLie}%
   {производная правого сдвига}%
   {derivative of right shift, 1-Parameter Group}%
\Symb{texLie}%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
\Symb{texVectorSpace}%
   {\drc вектор}%
   {drc vector}%
\Symb{texAffine}%
   {производная}%
   {overline nabla_l, definition 2}%
\Symb{texPolymodule}%
   {пассивное преобразование}%
   {passive transformation}%
\Symb{texBiring}%
   {\sups строка ($r$\hyph строка) матрицы}%
   {r row}%
\Symb{texBiring}%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
\Symb{texBiring}%
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Symb{texBiring}%
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Symb{texBiring}%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
\Symb{texTstarRepresentation}%
   {правый сдвиг}%
   {right shift}%
\Symb{texFiberedGroup}%
   {\sT сдвиг}%
   {starT shift, fibered group}%
\Symb{texTstarRepresentation}%
   {левый сдвиг}%
   {Tstar shift}%
\Symb{texFiberedGroup}%
   {\Ts сдвиг}%
   {Tstar shift, fibered group}%
\Symb{texReferenceFrame}%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Symb{texReferenceFrame}%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%

\SetIndexSpace%
\Symb{texBasis}%
   {многообразие базисов аффинного пространства}%
   {BAn}%
\Symb{texReferenceFrame}%
   {многообразие базисов многообразия}%
   {basis manifold of manifold}%
\Symb{texPolymodule}%
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Symb{texBasis}%
   {многообразие базисов векторного пространства $\mathcal{V}$}%
   {basis manifold of vector space}%
\Symb{texBasis}%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
\Symb{texBasis}%
   {многообразие базисов евклидова пространства}%
   {BEn}%
\Symb{texCartesian}%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Symb{texTypeBasis}%
   {многообразие базисов аффинного пространства}%
   {FAn}%
\Symb{texTypeBasis}%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
\Symb{texTypeBasis}%
   {многообразие базисов евклидова пространства}%
   {FEn}%

\SetIndexSpace%
\Symb{texBasis}%
   {центро-аффинное пространство}%
   {CAn}%
\Symb{texTypeBasis}%
   {центро-аффинное пространство}%
   {central affine space}%
\Symb{texLie}%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Symb{texLie}%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Symb{texReferenceFrame}%
   {множество функций, определённых на многообразии}%
   {set of functions defined on manifold}%

\SetIndexSpace%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of starT representation}%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of starT representation, coordinates}%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of Tstar representation}%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of Tstar representation, coordinates}%
\Symb{texVectorSpace}%
   {\dcr векторное пространство \subs строк}%
   {c rows dcr vector space}%
\Symb{texCalculus}%
   {дифференциал функции}%
   {differential, drc vector space to drc vector space}%
\Symb{texCalculus}%
   {дифференциал функции}%
   {differential, drc vector space to skew field}%
\Symb{texVectorSpace}%
   {\drc координатное векторное пространство}%
   {drc coordinate vector space}%
\Symb{texVectorSpace}%
   {векторное пространство матриц}%
   {matrices vector space}%
\Symb{texAffine}%
   {производная Картана}%
   {overbrace D}%
\Symb{texAffine}%
   {производная}%
   {overline D}%
\Symb{texCalculus}%
   {частная производная отображения $\Vector f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping, 1, drc vector space}%
\Symb{texCalculus}%
   {частная производная отображения $f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping, 1, skew field}%
\Symb{texVectorSpace}%
   {\drc векторное пространство \sups строк}%
   {r rows drc vector space}%
\Symb{texTidal}%
   {скорость отклонения}%
   {speed of deviation}%
\Symb{texVectorSpace}%
   {тип векторного пространства}%
   {vector space type}%

\SetIndexSpace%
\Symb{texTypeBasis}%
   {аффинный базис}%
   {Affine Basis}%
\Symb{texBasis}%
   {аффинный базис}%
   {Affine Basis}%
\Symb{texTypeBasis}%
   {базис}%
   {basis}%
\Symb{texBasis}%
   {базис векторного пространства}%
   {Basis e}%
\Symb{texBasis}%
   {базис в векторном пространстве $\mathcal{V}$}%
   {basis in V}%
\Symb{texVectorSpace}%
   {базис в векторном пространстве}%
   {basis, vector space}%
\Symb{texPolymodule}%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
\Symb{texCartesian}%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
\Symb{texCartesian}%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
\Symb{texBasis}%
   {центро-аффинный базис}%
   {Central Affine Basis}%
\Symb{texReferenceFrame}%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
\Symb{texTypeBasis}%
   {евклидово пространство}%
   {En}%
\Symb{texBasis}%
   {евклидово пространство}%
   {En}%
\Symb{texBasis}%
   {псевдоевклидово пространство}%
   {Enm}%
\Symb{texTypeBasis}%
   {псевдоевклидово пространство}%
   {Enm}%
\Symb{texFiberedAlgebra}%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
\Symb{texBasis}%
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Symb{texCartesian}%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
\Symb{texFiberedAlgebra}%
   {множество невырожденных \sT преобразований расслоения $\mathcal{E}$}%
   {set of starT nonsingular transformations of bundle}%
\Symb{texFiberedAlgebra}%
   {множество невырожденных \Ts преобразований расслоения $\mathcal{E}$}%
   {set of Tstar nonsingular transformations of bundle}%
\Symb{texBasis}%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Symb{texReferenceFrame}%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
\Symb{texReferenceFrame}%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
\Symb{texReferenceFrame}%
   {векторное поле системы отсчёта}%
   {vector field, reference frame}%
\Symb{texBasis}%
   {вектор базиса}%
   {vector of basis}%

\SetIndexSpace%
\Symb{texVectorSpace}%
   {координаты базиса в \dcr векторном пространстве \subs строк}%
   {basis coordinates, c rows dcr vector space}%
\Symb{texVectorSpace}%
   {координаты базиса в \drc векторном пространстве \sups строк}%
   {basis coordinates, r rows drc vector space}%
\Symb{texVectorSpace}%
   {базис в \dcr векторном пространстве \subs строк}%
   {basis, c rows dcr vector space}%
\Symb{texVectorSpace}%
   {базис в \drc векторного пространства \sups строк}%
   {basis, r rows drc vector space}%
\Symb{texDiffEq}%
   {центро-аффинный}%
   {Central Affine Basis}%
\Symb{texReferenceFrame}%
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Symb{texFiberedAlgebra}%
   {гомоморфизм расслоенных $\mathcal{F}$\Hyph алгебр}%
   {homomorphism of fibered F-algebras}%
\Symb{texBundleRelation}%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
\Symb{texBundleRelation}%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
\Symb{texCartesian}%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
\Symb{texTstarRepresentation}%
   {орбита представления группы $G$}%
   {orbit of representation of group}%
\Symb{texTypeBasis}%
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Symb{texReferenceFrame}%
   {система отсчёта}%
   {reference frame}%
\Symb{texReferenceFrame}%
   {система отсчёта}%
   {reference frame, extensive definition}%
\Symb{texPolymodule}%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Symb{texPolymodule}%
   {вектор базиса}%
   {vector of basis}%

\SetIndexSpace%
\Symb{texVectorSpace}%
   {\CR матричная группа}%
   {cr-matrix group}%
\Symb{texLie}%
   {алгебра Ли группы Ли}%
   {g}%
\Symb{texLie}%
   {определённая слева алгебра Ли группы Ли}%
   {gl}%
\Symb{texTypeBasis}%
   {группа аффинных преобразований}%
   {GLAn}%
\Symb{texBasis}%
   {группа аффинных преобразований}%
   {GLAn}%
\Symb{texLie}%
   {определённая справа алгебра Ли группы Ли}%
   {gr}%
\Symb{texBasis}%
   {группа гомоморфизмов векторного пространства $\mathcal{V}$}%
   {GV}%
\Symb{texFiberedGroup}%
   {орбита ковариантного эффективного \sT представления расслоенной группы}%
   {orbit of effective starT covariant representation of fibered group}%
\Symb{texTstarRepresentation}%
   {орбита ковариантного эффективного \sT представления группы}%
   {orbit of effective starT covariant representation of group}%
\Symb{texFiberedGroup}%
   {орбита ковариантного эффективного		\Ts представления расслоенной группы}%
   {orbit of effective Tstar covariant representation of fibered group}%
\Symb{texTstarRepresentation}%
   {орбита ковариантного эффективного		\Ts представления группы}%
   {orbit of effective Tstar covariant representation of group}%
\Symb{texVectorSpace}%
   {\RC матричная группа}%
   {rc-matrix group}%

\SetIndexSpace%
\Symb{texBiring}%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Symb{texLinearMap}%
   {\rcd векторное пространство \drc линейных отображений}%
   {rcd vector space of drc linear maps}%

\SetIndexSpace%
\Symb{texLieRepresentation}%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator of representation}%
\Symb{texLinearLie}%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%

\SetIndexSpace%
\Symb{texRepresentation}%
   {левый сдвиг}%
   {left shift}%
\Symb{texDiffProperty}%
   {производная Ли связности}%
   {Lie derivative of connection}%
\Symb{texDiffProperty}%
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Symb{texBasis}%
   {пассивное преобразование}%
   {passive transformation}%
\Symb{texRepresentation}%
   {множество левосторонних невырожденных преобразований множества $M$}%
   {set of left-side nonsingular transformations}%

\SetIndexSpace%
\Symb{texTstarMorphism}%
   {множество \sT преобразований множества $M$}%
   {set of starT transformations}%
\Symb{texTstarMorphism}%
   {множество \Ts преобразований множества $M$}%
   {set of Tstar transformations}%

\SetIndexSpace%
\Symb{texBasis}%
   {геометрический объект в координатном представлении}%
   {geometrical object, coordinate vector space}%
\Symb{texBasis}%
   {геометрический объект}%
   {geometrical object, vector space}%
\Symb{texFiberedGroup}%
   {орбита представления расслоенной группы $\mathcal{G}$}%
   {orbit of representation of fibered group}%
\Symb{texRepresentation}%
   {орбита представления группы $G$}%
   {orbit of representation of group}%

\SetIndexSpace%
\Symb{texCartesian}%
   {расслоение}%
   {bundle}%
\Symb{texCartesian}%
   {декартова степень расслоения}%
   {Cartesian power of bundle}%
\Symb{texCartesian}%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
\Symb{texCartesian}%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
\Symb{texFiberedAlgebra}%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
\Symb{texFiberedAlgebra}%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%

\SetIndexSpace%
\Symb{texBasis}%
   {активное преобразование}%
   {active transformation}%
\Symb{texAffine}%
   {кривизна Картана}%
   {Cartan curvature}%
\Symb{texVectorSpace}%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
\Symb{texBundleRelation}%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
\Symb{texBundleRelation}%
   {диагональ в расслоении $\mathcal{A}$}%
   {diagonal in reduced bundle, 2}%
\Symb{texAffine}%
   {кривизна}%
   {GLn curvature_overline}%
\Symb{texVectorSpace}%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Symb{texRepresentation}%
   {правый сдвиг}%
   {right shift}%
\Symb{texRepresentation}%
   {множество правосторонних невырожденных преобразований множества $M$}%
   {set of right-side nonsingular transformations}%

\SetIndexSpace%
\Symb{texBundleRelation}%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Symb{texBundleRelation}%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
\Symb{texBundleRelation}%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
\Symb{texVectorSpace}%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%

\SetIndexSpace%
\Symb{texLie}%
   {касательная плоскость к группе $G$}%
   {TaG}%

\SetIndexSpace%
\Symb{texBasis}%
   {координатное векторное пространство}%
   {coordinate vector space}%
\Symb{texBasis}%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
\Symb{texVectorSpace}%
   {\dcr векторное пространство}%
   {left CR vector space}%
\Symb{texVectorSpace}%
   {\drc векторное пространство}%
   {left RC vector space}%
\Symb{texLinearMap}%
   {($S$, $T$)\hyph бимодуль}%
   {R S bimodule}%
\Symb{texVectorSpace}%
   {\crd векторное пространство}%
   {right CR vector space}%
\Symb{texVectorSpace}%
   {\rcd векторное пространство}%
   {right RC vector space}%
\Symb{texBasis}%
   {векторное пространство}%
   {V}%
\Symb{texReferenceFrame}%
   {векторное пространство векторных полей}%
   {vector space of vector fields}%

\SetIndexSpace%
\Symb{texPolymodule}%
   {геометрический объект в координатном представлении,		определённом в векторном пространстве}%
   {geometrical object, coordinate vector space}%
\Symb{texPolymodule}%
   {геометрический объект в векторном пространстве}%
   {geometrical object, vector space}%

\SetIndexSpace%
\Symb{texReferenceFrame}%
   {неголономная координата}%
   {x(k)}%

\SetIndexSpace%
\Symb{texBundleRelation}%
   {диагональ в расслоении $\mathcal{A}$}%
   {diagonal in bundle, 1}%

\SetIndexSpace%
\Symb{texTidal}%
   {отклонение траекторий}%
   {deviation of trajectories}%
\Symb{texRepresentation}%
   {тождественное преобразование}%
   {identical transformation}%
\Symb{texTstarMorphism}%
   {тождественное преобразование}%
   {identical transformation}%
\Symb{texBasis}%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
\Symb{texBiring}%
   {символ Кронекерa}%
   {Kronecker symbol}%

\SetIndexSpace%
\Symb{texReferenceFrame}%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Symb{texAffine}%
   {символ Картана}%
   {Cartan symbol}%
\Symb{texAffine}%
   {связность}%
   {conection overline}%
\Symb{texAffine}%
   {связность Картана}%
   {overbrace Gamma i kl}%
\Symb{texCartesian}%
   {множество сечений расслоения}%
   {set of sections of bundle}%

\SetIndexSpace%
\Symb{texLie}%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
\Symb{texLie}%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%

\SetIndexSpace%
\Symb{texReferenceFrame}%
   {объект неголономности}%
   {anholonomity object}%

\SetIndexSpace%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%

\SetIndexSpace%
\Symb{texReferenceFrame}%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
\Symb{texCalculus}%
   {частная производная отображения $\Vector f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping, 2, drc vector space}%
\Symb{texCalculus}%
   {частная производная отображения $f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping, 2, skew field}%
\Symb{texReferenceFrame}%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%

\SetIndexSpace%
\Symb{texLie}%
   {операция на группе Ли}%
   {Lie group composition law}%

\SetIndexSpace%
\Symb{texAffine}%
   {производная Картана}%
   {overbrace nabla_l}%
\Symb{texAffine}%
   {производная Картана}%
   {overbrace nabla_l}%
\Symb{texAffine}%
   {производная}%
   {overline nabla_l, definition 1}%

\SetIndexSpace%
\Symb{texBundleRelation}%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%

\SetIndexSpace%
\Symb{texCartesian}%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
\Symb{texCartesian}%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
\Symb{texCartesian}%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
\Symb{texCartesian}%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%

\SetIndexSpace%
\Symb{texBundleRelation}%
   {расслоенное подмножество}%
   {fibered subset}%
\Symb{texBundleRelation}%
   {подрасслоение}%
   {subbundle}%

\CloseIndex

